Deep Reinforcement Learning for Sim-to-Real Policy Transfer of VTOL-UAVs Offshore Docking Operations

This paper proposes a novel Reinforcement Learning (RL) approach for sim-to-real policy transfer of Vertical Take-Off and Landing Unmanned Aerial Vehicle (VTOL-UAV). The proposed approach is designed for VTOL-UAV landing on offshore docking stations in maritime operations. VTOL-UAVs in maritime operations encounter limitations in their operational range, primarily stemming from constraints imposed by their battery capacity. The concept of autonomous landing on a charging platform presents an intriguing prospect for mitigating these limitations by facilitating battery charging and data transfer. However, current Deep Reinforcement Learning (DRL) methods exhibit drawbacks, including lengthy training times, and modest success rates. In this paper, we tackle these concerns comprehensively by decomposing the landing procedure into a sequence of more manageable but analogous tasks in terms of an approach phase and a landing phase. The proposed architecture utilizes a model-based control scheme for the approach phase, where the VTOL-UAV is approaching the offshore docking station. In the Landing phase, DRL agents were trained offline to learn the optimal policy to dock on the offshore station. The Joint North Sea Wave Project (JONSWAP) spectrum model has been employed to create a wave model for each episode, enhancing policy generalization for sim2real transfer. A set of DRL algorithms have been tested through numerical simulations including value-based agents and policy-based agents such as Deep \textit{Q} Networks (DQN) and Proximal Policy Optimization (PPO) respectively. The numerical experiments show that the PPO agent can learn complicated and efficient policies to land in uncertain environments, which in turn enhances the likelihood of successful sim-to-real transfer.

==> docs/c1ef8079-0aee-47bd-8767-31342f7fa5ef <==
{"id":"r0.028598576954188437","lines":[{"id":"n0.34271031921238304","blocks":[]},{"blocks":[],"id":"n0.7182255252531358"},{"id":"n0.754108336679199","blocks":[{"id":"n0.38980013235984456","text":"\\diagram","type":"composite","elements":{"de23639326403757055":{"id":"de23639326403757055","lines":[{"blocks":[{"text":"r","id":"n0.8662818617344707"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"t","id":"n0.6132178761850728"}],"id":"n0.335979536439849"}],"id":"n0.9227737368848539"}},"id":"n0.2700860069638791"},{"text":",s","id":"n0.14372035682465656"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"t","id":"n0.04375871319597935"}],"id":"n0.17392585219789125"}],"id":"n0.41032008023294764"}},"id":"n0.7074221172209534"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"+","id":"n0.9335995514640594"}],"id":"n0.6572681880937001"}],"id":"n0.9212104885783379"}},"id":"n0.5054471570619099"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.20027857312308628"}],"id":"n0.07037625209572984"}],"id":"n0.2319737794531127"}},"id":"n0.3732966687187318"}],"id":"n0.13345289084323309"}],"shape":{"data":{"p":{"x":129.08530525523946,"y":297.5309009625462},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"},"style":{"textColor":[245,166,35,1]}},"isMathDisplayMode":true},"de46988013856580246":{"id":"de46988013856580246","lines":[{"blocks":[{"text":"s","id":"n0.24333901291683713"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"t","id":"n0.1664433885118748"}],"id":"n0.4357623342582839"}],"id":"n0.777068199589436"}},"id":"n0.8188362313553208"}],"id":"n0.7441557146445386"}],"shape":{"data":{"p":{"x":136.8283791606585,"y":181.92866204531344},"rotation":0},"anchor":"left-top","style":{"textColor":[245,166,35,1]}},"isMathDisplayMode":true},"de2188706979097701":{"id":"de2188706979097701","lines":[{"blocks":[{"text":"memory list","id":"n0.8181348941803446"}],"id":"n0.6612853737178506"}],"shape":{"data":{"p":{"x":170.61563357445763,"y":323.6831744914012},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de39973677978740363":{"id":"de39973677978740363","lines":[{"blocks":[{"text":"Experinece buffer","id":"n0.6358277625350996"}],"id":"n0.1631933610395575"}],"shape":{"data":{"p":{"x":244.61418685249356,"y":354.41721997025525},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de19978742928587212":{"id":"de19978742928587212","lines":[{"blocks":[{"text":"Mini Batch","id":"n0.4748088058836799"}],"id":"n0.858918731872411"}],"shape":{"data":{"p":{"x":265.35228668309094,"y":225.44816369681047},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de89400025535266":{"id":"de89400025535266","lines":[{"blocks":[{"text":"Hidden ","id":"n0.12704521553190018"}],"id":"n0.8038535701302112"},{"blocks":[{"text":"Layers","id":"n0.5642507574936066"}],"style":null,"id":"n0.9371407862413408"}],"shape":{"data":{"p":{"x":409.8853616693237,"y":109.56082636068382},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de2556569085184557":{"id":"de2556569085184557","lines":[{"blocks":[{"text":"s","id":"n0.32153617574000437"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"t","id":"n0.9432576686820728"}],"id":"n0.12070453188665686"}],"id":"n0.6370001195703945"}},"id":"n0.8734101275148849"}],"id":"n0.02023333726124754"}],"shape":{"data":{"p":{"x":378.1719212603528,"y":117.87703047368048},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de3914138980260946":{"id":"de3914138980260946","lines":[{"blocks":[{"id":"n0.34827830730387244","text":"a"},{"id":"n0.08878403942123403","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6629482314459245","lines":[{"id":"n0.7765478462824684","blocks":[{"id":"n0.051593690421772864","text":"1"}]}]}}}],"id":"n0.1938583513253611"}],"shape":{"data":{"p":{"x":486.076920242896,"y":97.33700214499352},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\tiny"}},"isMathDisplayMode":true},"de806707849619654":{"id":"de806707849619654","lines":[{"blocks":[{"id":"n0.5448976978364997","text":"Critic Nueral Network"}],"id":"n0.5608582563569307"}],"shape":{"data":{"p":{"x":379.7432440182633,"y":305.083024102163},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de7134260069953413":{"id":"de7134260069953413","lines":[{"blocks":[{"text":"Actor Nueral Network","id":"n0.7142153424964763"}],"id":"n0.1115056452272809"}],"shape":{"data":{"p":{"x":380.22789641729696,"y":174.6089319554142},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de643099887539367":{"id":"de643099887539367","lines":[{"blocks":[{"text":"Hidden ","id":"n0.3934590587825675"}],"id":"n0.5876089366784423"},{"blocks":[{"text":"Layers","id":"n0.9540403541356623"}],"style":null,"id":"n0.7366818034814431"}],"shape":{"data":{"p":{"x":407.9822921491304,"y":234.13911169073899},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de9704691071265719":{"id":"de9704691071265719","lines":[{"blocks":[{"text":"s","id":"n0.4073150962358092"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"t","id":"n0.4272995328523337"}],"id":"n0.6422019552330569"}],"id":"n0.3773963049056277"}},"id":"n0.9094381183534617"}],"id":"n0.6601689055491329"}],"shape":{"data":{"p":{"x":376.26885174015956,"y":242.4553158037357},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de8467359976366438":{"id":"de8467359976366438","lines":[{"blocks":[{"id":"n0.13744813804330436","text":"a"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.8115265678962766"}],"id":"n0.37149573760369003"}],"id":"n0.6596707367462691"}},"id":"n0.16486218031026278"}],"id":"n0.1654491083925349"}],"shape":{"data":{"p":{"x":484.22231596260616,"y":222.7925993435702},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\tiny"}},"isMathDisplayMode":true},"de3911015067597048":{"id":"de3911015067597048","lines":[{"blocks":[{"id":"n0.9597982520688293","text":"a"},{"id":"n0.42021846739666024","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5584176966488825","lines":[{"id":"n0.881266238629459","blocks":[{"id":"n0.0910031437428307","text":"n"}]}]}}}],"id":"n0.9245787922473896"}],"shape":{"data":{"p":{"x":484.22231596260616,"y":263.14894529555994},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\tiny"}},"isMathDisplayMode":true},"de7232305177292":{"id":"de7232305177292","lines":[{"blocks":[{"text":"a","id":"n0.6820969539468476"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"t","id":"n0.1837435747418492"}],"id":"n0.7351943334649464"}],"id":"n0.8920275528939843"}},"id":"n0.6012853175270572"}],"id":"n0.3642774122734025"}],"shape":{"data":{"p":{"x":85.42126949548826,"y":145.08156356740977},"rotation":0},"anchor":"left-top","style":{"textColor":[65,117,5,1]}},"isMathDisplayMode":true},"de03699718944736552":{"id":"de03699718944736552","lines":[{"blocks":[{"text":"Docking Phase","id":"n0.7695468671990482"}],"id":"n0.8207025954859106"},{"blocks":[{"text":" Envirmoent ","id":"n0.29964516542811315"}],"style":null,"id":"n0.4606958531594334"}],"shape":{"data":{"p":{"x":25.80645978444693,"y":227.83660078876184},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de10764678373358683":{"id":"de10764678373358683","lines":[{"blocks":[{"text":"PPO Learning Architecture","id":"n0.30011617170660077"}],"id":"n0.6479768290984376"}],"shape":{"data":{"p":{"x":176.1683396256592,"y":68.77928137523845},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\small"},"style":{"textColor":[20,60,120,1],"strokeType":"--","strokeColor":[20,60,120,1]},"frameType":"rectangle"},"isMathDisplayMode":true},"de5025052513560613":{"id":"de5025052513560613","lines":[{"blocks":[{"text":"DRL Agent ","id":"n0.7952220601264208"}],"id":"n0.6259203917834804"}],"shape":{"data":{"p":{"x":150.65979803337098,"y":13.918380679934039},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\small"},"style":{"textColor":[208,2,27,1]}},"isMathDisplayMode":true},"de21377130484944895":{"id":"de21377130484944895","lines":[{"blocks":[{"text":"Envirmoent","id":"n0.37246229730675595"}],"id":"n0.05800258449175777"}],"shape":{"data":{"p":{"x":25.854635407894875,"y":13.593755233318454},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\small"},"style":{"textColor":[208,2,27,1]}},"isMathDisplayMode":true},"de809236258541969":{"id":"de809236258541969","lines":[{"blocks":[{"text":"a","id":"n0.2477448913335285"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.4830361225876576","text":"n"}],"id":"n0.1723059157715563"}],"id":"n0.8298928965984516"}},"id":"n0.23194048576976756"}],"id":"n0.2064821947428772"}],"shape":{"data":{"p":{"x":486.076920242896,"y":138.3370021449935},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\tiny"}},"isMathDisplayMode":true},"de23894334541707796":{"id":"de23894334541707796","lines":[{"id":"n0.8690254046734942","blocks":[{"id":"n0.8999017666071119","text":"b"},{"id":"n0.7656385202989129","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.8937508636355127","lines":[{"id":"n0.7070984345779074","blocks":[{"id":"n0.01272936578246675","text":"t"}]}]}}},{"id":"n0.682515876756915","type":"single","text":"("},{"id":"n0.16239761187417967","text":"𝜃"},{"id":"n0.2785068416675356","type":"single","text":")"}]}],"shape":{"data":{"p":{"x":522.0768541134513,"y":118.41674991590497}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de7164229811408027":{"id":"de7164229811408027","lines":[{"blocks":[{"id":"n0.7036470758525306","text":"A"},{"id":"n0.137447264990336","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.06300417802204583","lines":[{"id":"n0.49061173013613235","blocks":[{"id":"n0.7449312758954212","text":"t"}]}]}}}],"id":"n0.8587899691233101"}],"shape":{"data":{"p":{"x":534.0768541134513,"y":241.41674991590497}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de15258933700620214":{"id":"de15258933700620214","lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"id":"n0.09892539685977186","text":"L"},{"id":"n0.030364806545160716","text":"\\power","type":"composite","elements":{"powerValue":{"id":"n0.17945836112343927","lines":[{"id":"n0.38335004825450514","blocks":[{"id":"n0.04991483545236908","text":"VF"}]}]}},"style":{}}],"id":"n0.24732977568627867"}],"shape":{"data":{"p":{"x":535.0768541134513,"y":278.416749915905}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de3432748431252459":{"id":"de3432748431252459","lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"text":"L","id":"n0.42493440126106985"},{"text":"\\power","type":"composite","elements":{"powerValue":{"lines":[{"blocks":[{"id":"n0.3437861605703245","text":"clip"}],"id":"n0.13687209231200326"}],"id":"n0.32002257845321047"}},"style":{},"id":"n0.8453746909764885"},{"id":"n0.3226828330447913","type":"single","text":"("},{"id":"n0.7784111005611898","text":"𝜃"},{"id":"n0.9403089682545536","type":"single","text":")"}],"id":"n0.5934311315827032"}],"shape":{"data":{"p":{"x":585.0768541134513,"y":178.41674991590497}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de7781601700991372":{"id":"de7781601700991372","lines":[{"id":"n0.0227045959417711","blocks":[{"id":"n0.40778794021852893","text":"update weights of critic"}]},{"id":"n0.49147571174076154","blocks":[{"text":" NN  based on SGD","id":"n0.848528246096039"}],"style":null}],"shape":{"data":{"p":{"x":518.5714416503906,"y":337}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"},"style":{"textColor":[144,19,254,1]}},"isMathDisplayMode":true},"de6861159344954277":{"id":"de6861159344954277","lines":[{"blocks":[{"text":"update weights of Actor","id":"n0.531247825912537"}],"id":"n0.09495438377163223"},{"blocks":[{"text":" NN  based on SGD","id":"n0.5225477213106755"}],"style":null,"id":"n0.164515699999785"}],"shape":{"data":{"p":{"x":518.5714416503906,"y":71}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"},"style":{"textColor":[144,19,254,1]}},"isMathDisplayMode":true},"de6311410765902101":{"id":"de6311410765902101","lines":[{"id":"n0.3584111210090346","blocks":[{"id":"n0.8160260449154462","text":"\\frac","type":"composite","elements":{"value":{"id":"n0.9433832361386592","lines":[{"id":"n0.46988884786736196","blocks":[{"id":"n0.5463168578634294","text":"𝜋"},{"id":"n0.1845896996511136","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.37051079986290714","lines":[{"id":"n0.3720035770149257","blocks":[{"id":"n0.45251688327586503","text":"𝜃"}]}]}}},{"id":"n0.8804368311172961","type":"single","text":"("},{"id":"n0.9866138922444603","text":"a"},{"id":"n0.24949685805026367","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.252261728365637","lines":[{"id":"n0.595802057442564","blocks":[{"id":"n0.8712461498345778","text":"t"}]}]}}},{"id":"n0.3410847779638224","text":"|s"},{"id":"n0.711639905906186","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6424471116273021","lines":[{"id":"n0.04922343732414891","blocks":[{"id":"n0.7484313419989743","text":"t"}]}]}}},{"id":"n0.4295230739653111","type":"single","text":")"}]}]},"sub1":{"id":"n0.4911179488746167","lines":[{"id":"n0.49474257013245393","blocks":[{"id":"n0.3644741212381064","text":"𝜋"},{"id":"n0.24838436567696265","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.08309428414977482","lines":[{"id":"n0.03970040426508903","blocks":[{"id":"n0.4669708252143885","text":"o"}]}]}}},{"id":"n0.053748749287670705","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.2443498164692839","lines":[{"id":"n0.2310268918140712","blocks":[{"id":"n0.7063617214277296","text":"l"}]}]}}},{"id":"n0.15735462291996938","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.09847576102154076","lines":[{"id":"n0.3497049105272583","blocks":[{"id":"n0.8958058832408509","text":"d"}]}]}}},{"id":"n0.5226763712411904","type":"single","text":"("},{"id":"n0.6749502676133627","text":"a"},{"id":"n0.0387155300441171","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.63451643599663","lines":[{"id":"n0.8007957220657902","blocks":[{"id":"n0.34779051142688133","text":"t"}]}]}}},{"id":"n0.13957038887131823","text":"|s"},{"id":"n0.20849477117447335","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.6603397055017164","lines":[{"id":"n0.9895728086249194","blocks":[{"id":"n0.6426325302303642","text":"t"}]}]}}},{"id":"n0.8984310438297523","type":"single","text":")"}]}]}}}]}],"shape":{"data":{"p":{"x":505.81422934419237,"y":138.68132979064194}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de3091806843543985":{"id":"de3091806843543985","lines":[{"id":"n0.8122195871304503","blocks":[{"id":"n0.962356762632131","text":"𝛿"},{"id":"n0.5995592686509306","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9865571025270532","lines":[{"id":"n0.6572239165186005","blocks":[{"id":"n0.3607034431641103","text":"t"}]}]}}}]}],"shape":{"data":{"p":{"x":510.5714416503906,"y":229}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de2684893218248463":{"id":"de2684893218248463","lines":[{"blocks":[{"text":"\\frac","type":"composite","elements":{"value":{"lines":[{"blocks":[{"id":"n0.9168691960073982","text":"V"},{"id":"n0.4635252789405555","type":"single","text":"("},{"id":"n0.9715730602108286","text":"s"},{"id":"n0.31510774855801826","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.22430387742386748","lines":[{"id":"n0.7763435465737694","blocks":[{"id":"n0.14963398775607017","text":"t"}]}]}}},{"id":"n0.6445642170915917","type":"single","text":")"}],"id":"n0.5575255911773889"}],"id":"n0.058939014049227634"},"sub1":{"lines":[{"blocks":[{"id":"n0.3755885134225665","text":"V"},{"id":"n0.2851473037621153","type":"single","text":"("},{"id":"n0.5080959257674236","text":"s"},{"id":"n0.45836528606206106","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.32367854079969693","lines":[{"id":"n0.4646309993584681","blocks":[{"id":"n0.38126785327668133","text":"t+1"}]}]}}},{"id":"n0.8849408179183602","type":"single","text":")"}],"id":"n0.9586758757410752"}],"id":"n0.7520782849759102"}},"id":"n0.47606393241159006"}],"id":"n0.5670870731039652"}],"shape":{"data":{"p":{"x":492.8142293441924,"y":289.68132979064194}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true}},"connections":[],"intersections":{"id":"di9061267162051334","items":[],"style":{}},"shapes":[{"id":"dp7773359347534068","type":"image","data":{"p1":{"x":35.28464960149941,"y":169.47469267358926},"p2":{"x":101.40790577552963,"y":229.67692276093908},"url":"data-resources/b663c298-b148-4425-918a-23e2f39d533f"}},{"id":"dp41737945127501486","type":"rectangle","data":{"p1":{"x":4.33331298828125,"y":171.0183395989059},"p2":{"x":134.3288546338139,"y":226.58962891030578}},"style":{"thickness":2}},{"id":"dp48812470623663606","type":"ellipse","data":{"p1":{"x":248.91017188992953,"y":273.93106518885156},"p2":{"x":334.8422890349717,"y":302.95162031855}},"style":{"thickness":2}},{"id":"da7967321713703379","data":[{"x":248.91017188992953,"y":287.6695192910424},{"x":248.91016866984097,"y":336.14003583747217}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da3624797965316906","data":[{"x":334.8422890349717,"y":288.4413427537007},{"x":335.0111118376613,"y":336.14003583747217}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"dp4343156777665489","type":"ellipse","data":{"p1":{"x":248.91016866984097,"y":321.6297582726229},"p2":{"x":335.0111118376613,"y":350.6503134023213}},"style":{"thickness":2}},{"id":"da8261580321035924","data":[{"x":107.05376696196562,"y":226.19605519855187},{"x":107.3730864127061,"y":317.0888240797424}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[245,166,35,1]}},{"id":"da3831373296076177","data":[{"x":107.3730864127061,"y":317.0888240797424},{"x":190.5169670728813,"y":316.935170369451}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[245,166,35,1]}},{"id":"da5426090040753779","data":[{"x":138.18255526756613,"y":204.639251198697},{"x":202.88691895413757,"y":204.639251198697}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[245,166,35,1]}},{"id":"da5505044926259","data":[{"x":202.88691895413757,"y":204.639251198697},{"x":202.88691895413757,"y":312.7992639111543}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[245,166,35,1]}},{"id":"dp13005115432085157","type":"rectangle","data":{"p1":{"x":192.0768541134513,"y":312.416749915905},"p2":{"x":215.8812323576678,"y":322.1417184791451}}},{"id":"da959400337301765","data":[{"x":214.62250948890673,"y":317.52003602398753},{"x":249.18640457146887,"y":317.7551591365375}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[7,144,226,1]}},{"id":"dp2767158234618814","type":"rectangle","data":{"p1":{"x":262.4162017882531,"y":331.8178248882264},"p2":{"x":286.2205800324695,"y":342.31461691412477}}},{"id":"dp8979821608807763","type":"rectangle","data":{"p1":{"x":296.1812775403394,"y":331.0460014255681},"p2":{"x":319.98565578455595,"y":341.54279345146654}}},{"id":"dp9511030094288098","type":"rectangle","data":{"p1":{"x":295.3371506465372,"y":307.8912975458182},"p2":{"x":319.1415288907537,"y":318.38808957171653}}},{"id":"dp8365112248516693","type":"rectangle","data":{"p1":{"x":260.72794800064867,"y":307.1194740831598},"p2":{"x":284.5323262448652,"y":317.61626610905824}}},{"id":"dp22369672176642652","type":"rectangle","data":{"p1":{"x":259.88382110684654,"y":284.7365936660682},"p2":{"x":283.6881993510631,"y":295.23338569196665}}},{"id":"dp6823554345447072","type":"rectangle","data":{"p1":{"x":293.64889685893297,"y":284.7365936660682},"p2":{"x":317.4532751031494,"y":295.23338569196665}}},{"id":"da5192546933090174","data":[{"x":291.8762304624506,"y":273.93106518885156},{"x":291.37965164312504,"y":259.3250265676577}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"dp7860298064715456","type":"rectangle","data":{"p1":{"x":266.3297486949341,"y":246.53396953498833},"p2":{"x":290.1341269391505,"y":257.03076156088673}}},{"id":"dp6969145959148118","type":"rectangle","data":{"p1":{"x":298.40657065941616,"y":246.53396953498833},"p2":{"x":322.2109489036327,"y":257.03076156088673}}},{"id":"dp3615259117742271","type":"rectangle","data":{"p1":{"x":256.2002263718191,"y":242.67485222169668},"p2":{"x":332.17164681401357,"y":260.1180554115201}},"style":{"thickness":2}},{"id":"da5377253775007014","data":[{"x":333.7984824451342,"y":251.16491031093832},{"x":377.01778005182257,"y":251.62799732227845}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"dp9989994962719235","type":"ellipse","data":{"p1":{"x":379.87238433211246,"y":123.25175835791867},"p2":{"x":390.5534541703556,"y":133.1557197693769}}},{"id":"dp2142772976311218","type":"ellipse","data":{"p1":{"x":405.812125367846,"y":69.5081702059976},"p2":{"x":416.4931952060893,"y":79.41213161745586}}},{"id":"dp2355334708390835","type":"ellipse","data":{"p1":{"x":405.812125367846,"y":164.90668625750726},"p2":{"x":416.4931952060893,"y":174.8106476689655}}},{"id":"dp4987346479831327","type":"ellipse","data":{"p1":{"x":406.57505892772053,"y":84.65541216913998},"p2":{"x":417.2561287659637,"y":94.55937358059822}}},{"id":"dp174764446615002","type":"ellipse","data":{"p1":{"x":406.57505892772053,"y":149.46814444840987},"p2":{"x":417.2561287659637,"y":159.37210585986813}}},{"id":"da7714153036561029","data":[{"x":411.91559384684217,"y":94.55937358059822},{"x":411.91559384684217,"y":149.46814444840987}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"dp7398403084962235","type":"ellipse","data":{"p1":{"x":447.01053760106987,"y":69.5081702059976},"p2":{"x":457.69160743931303,"y":79.41213161745586}}},{"id":"dp40207518588260593","type":"ellipse","data":{"p1":{"x":447.01053760106987,"y":164.90668625750726},"p2":{"x":457.69160743931303,"y":174.8106476689655}}},{"id":"dp20872568288027482","type":"ellipse","data":{"p1":{"x":447.7734711609444,"y":84.65541216913998},"p2":{"x":458.45454099918766,"y":94.55937358059822}}},{"id":"dp7662590256237038","type":"ellipse","data":{"p1":{"x":447.7734711609444,"y":149.46814444840987},"p2":{"x":458.45454099918766,"y":159.37210585986813}}},{"id":"da772307539800835","data":[{"x":453.114006080066,"y":94.55937358059822},{"x":453.114006080066,"y":149.46814444840987}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da2600657060099054","data":[{"x":390.5534541703556,"y":128.2037390636478},{"x":405.812125367846,"y":74.46015091172674}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5313937734744587","data":[{"x":390.5534541703556,"y":128.2037390636478},{"x":407.33799248759505,"y":93.39420753263704}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da20435821953732636","data":[{"x":390.5534541703556,"y":128.2037390636478},{"x":405.812125367846,"y":169.85866696323637}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7310874496787376","data":[{"x":390.5534541703556,"y":128.2037390636478},{"x":406.57505892772053,"y":154.42012515413896}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6652535373397381","data":[{"x":416.4931952060893,"y":74.46015091172674},{"x":447.01053760106987,"y":74.46015091172674}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7652439859258313","data":[{"x":416.4931952060893,"y":74.46015091172674},{"x":447.7734711609444,"y":89.6073928748691}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da3698848742532972","data":[{"x":417.2561287659637,"y":89.6073928748691},{"x":447.01053760106987,"y":74.46015091172674}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6475484634614972","data":[{"x":417.2561287659637,"y":89.6073928748691},{"x":447.7734711609444,"y":89.6073928748691}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da340097150018869","data":[{"x":416.4931952060893,"y":169.85866696323637},{"x":447.01053760106987,"y":169.85866696323637}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da33485742259001294","data":[{"x":417.2561287659637,"y":154.42012515413896},{"x":447.7734711609444,"y":154.42012515413896}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8077609298648467","data":[{"x":417.2561287659637,"y":154.42012515413896},{"x":447.01053760106987,"y":169.85866696323637}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8272021155345739","data":[{"x":416.4931952060893,"y":169.85866696323637},{"x":447.7734711609444,"y":154.42012515413896}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp05095935613153979","type":"ellipse","data":{"p1":{"x":485.9201491546701,"y":99.36182697611515},"p2":{"x":498.81422934419237,"y":110.14356531267306}}},{"id":"da11395833077421225","data":[{"x":491.26068407379177,"y":110.14356531267306},{"x":491.26068407379177,"y":140.72934908491283}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da7289663156160691","data":[{"x":457.69160743931303,"y":74.46015091172674},{"x":485.9201491546701,"y":105.19158460694395}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da37617251649011973","data":[{"x":458.45454099918766,"y":89.6073928748691},{"x":485.9201491546701,"y":105.19158460694395}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da06709883175119713","data":[{"x":458.45454099918766,"y":154.42012515413896},{"x":485.9201491546701,"y":145.6813297906419}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7689062011022951","data":[{"x":457.69160743931303,"y":169.85866696323637},{"x":485.9201491546701,"y":145.6813297906419}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp7219078308048199","type":"ellipse","data":{"p1":{"x":377.9693148119192,"y":247.83004368797384},"p2":{"x":388.6503846501624,"y":257.7340050994321}}},{"id":"dp43895083411935953","type":"ellipse","data":{"p1":{"x":403.9090558476528,"y":194.08645553605282},"p2":{"x":414.590125685896,"y":203.99041694751105}}},{"id":"dp4138382232646227","type":"ellipse","data":{"p1":{"x":403.9090558476528,"y":289.4849715875624},"p2":{"x":414.590125685896,"y":299.3889329990206}}},{"id":"dp43010657639595395","type":"ellipse","data":{"p1":{"x":404.6719894075273,"y":209.23369749919513},"p2":{"x":415.35305924577045,"y":219.13765891065347}}},{"id":"dp8586680722575293","type":"ellipse","data":{"p1":{"x":404.6719894075273,"y":274.04642977846504},"p2":{"x":415.35305924577045,"y":283.9503911899234}}},{"id":"da4299337695604506","data":[{"x":410.0125243266489,"y":219.13765891065347},{"x":410.0125243266489,"y":274.04642977846504}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"dp5200555552211097","type":"ellipse","data":{"p1":{"x":445.1074680808766,"y":194.08645553605282},"p2":{"x":455.7885379191198,"y":203.99041694751105}}},{"id":"dp5584249970397268","type":"ellipse","data":{"p1":{"x":445.1074680808766,"y":289.4849715875624},"p2":{"x":455.7885379191198,"y":299.3889329990206}}},{"id":"dp9775140219880036","type":"ellipse","data":{"p1":{"x":445.870401640751,"y":209.23369749919513},"p2":{"x":456.5514714789943,"y":219.13765891065347}}},{"id":"dp07125179793933767","type":"ellipse","data":{"p1":{"x":445.870401640751,"y":274.04642977846504},"p2":{"x":456.5514714789943,"y":283.9503911899234}}},{"id":"da38640159876483593","data":[{"x":451.2109365598728,"y":219.13765891065347},{"x":451.2109365598728,"y":274.04642977846504}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da4244730605219442","data":[{"x":388.6503846501624,"y":252.78202439370304},{"x":403.9090558476528,"y":199.03843624178194}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da27862039630939606","data":[{"x":388.6503846501624,"y":252.78202439370304},{"x":405.4349229674017,"y":217.9724928626922}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da3295634387318367","data":[{"x":388.6503846501624,"y":252.78202439370304},{"x":403.9090558476528,"y":294.43695229329154}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9237090346684198","data":[{"x":388.6503846501624,"y":252.78202439370304},{"x":404.6719894075273,"y":278.99841048419415}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da854389951854315","data":[{"x":414.590125685896,"y":199.03843624178194},{"x":445.1074680808766,"y":199.03843624178194}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5119042051032991","data":[{"x":414.590125685896,"y":199.03843624178194},{"x":445.870401640751,"y":214.18567820492424}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da4084922304167917","data":[{"x":415.35305924577045,"y":214.18567820492424},{"x":445.1074680808766,"y":199.03843624178194}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da18605408270307544","data":[{"x":415.35305924577045,"y":214.18567820492424},{"x":445.870401640751,"y":214.18567820492424}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5910299795183522","data":[{"x":414.590125685896,"y":294.43695229329154},{"x":445.1074680808766,"y":294.43695229329154}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da49468192752037465","data":[{"x":415.35305924577045,"y":278.99841048419415},{"x":445.870401640751,"y":278.99841048419415}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5888344642360879","data":[{"x":415.35305924577045,"y":278.99841048419415},{"x":445.1074680808766,"y":294.43695229329154}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da07386338476205379","data":[{"x":414.590125685896,"y":294.43695229329154},{"x":445.870401640751,"y":278.99841048419415}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6835857828452236","data":[{"x":489.3576145535984,"y":234.72185064272833},{"x":489.3576145535984,"y":265.30763441496794}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da18106336253864175","data":[{"x":455.7885379191198,"y":199.03843624178194},{"x":484.0170796344769,"y":229.76986993699913}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da33813403088949556","data":[{"x":456.5514714789943,"y":214.18567820492424},{"x":484.0170796344769,"y":229.76986993699913}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8528136771712673","data":[{"x":456.5514714789943,"y":278.99841048419415},{"x":484.0170796344769,"y":270.25961512069705}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6500797470615316","data":[{"x":455.7885379191198,"y":294.43695229329154},{"x":484.0170796344769,"y":270.25961512069705}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp8503902729304145","type":"ellipse","data":{"p1":{"x":485.9201491546701,"y":140.29046062236296},"p2":{"x":498.81422934419237,"y":151.0721989589209}}},{"id":"dp02339559520977863","type":"ellipse","data":{"p1":{"x":484.0170796344769,"y":224.3790007687202},"p2":{"x":496.911159823999,"y":235.16073910527814}}},{"id":"dp11439302263522855","type":"ellipse","data":{"p1":{"x":484.0170796344769,"y":264.8687459524182},"p2":{"x":496.911159823999,"y":275.65048428897603}}},{"id":"da9263183815446665","data":[{"x":489.3576145535984,"y":250.0147425288481},{"x":526.3333129882812,"y":250.3333282470703}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da40635466998338043","data":[{"x":507.40740859024834,"y":125.5588201152768},{"x":508.5,"y":41.5}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[65,117,5,1]}},{"id":"da9824271145595218","data":[{"x":508.5,"y":41.5},{"x":79.18740014157446,"y":39.704619916652106}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[65,117,5,1]}},{"id":"da11489743305936728","data":[{"x":79.18740014157446,"y":39.704619916652106},{"x":79.18740014157446,"y":168.66946458931488}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[65,117,5,1]}},{"id":"dp7951418372825128","type":"rectangle","data":{"p1":{"x":170.53473711085186,"y":64.26934554189617},"p2":{"x":643.4285583496094,"y":370.451187655905}},"style":{"strokeColor":[20,60,200,1],"boxShadow":{"fill":[0,0,0,0.09]}}},{"id":"da6622843143643202","data":[{"x":126.62049038239462,"y":15.064473930377119},{"x":125.87178436913706,"y":171.43462392060707}],"head":"no","tail":"no","shaft":"--","mVer":1,"style":{"thickness":2,"strokeColor":[208,2,27,1]}},{"id":"da7586036474512297","data":[{"x":126.62049038239462,"y":228.29650650391068},{"x":125.87178436913706,"y":384.6666564941406}],"head":"no","tail":"no","shaft":"--","mVer":1,"style":{"thickness":2,"strokeColor":[208,2,27,1]}},{"id":"da5403383830180783","data":[{"x":355.4222459042348,"y":213.13333251276472},{"x":355.4081312484784,"y":251.39645381660836}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da41914995792351895","data":[{"x":355.4222459042347,"y":213.13333251276472},{"x":356.4704215276827,"y":127.8405194833513}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da3220888863231359","data":[{"x":356.4704215276827,"y":127.8405194833513},{"x":379.87238433211246,"y":128.2037390636478}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da4241044315135498","data":[{"x":491.26068407379177,"y":125.43645719879294},{"x":523.554133106705,"y":125.68118303176067}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"dp25622603355315277","type":"rectangle","data":{"p1":{"x":522.0768541134513,"y":118.41674991590497},"p2":{"x":555.4285583496094,"y":136.1428565979004}}},{"id":"dp47142694447147915","type":"rectangle","data":{"p1":{"x":528.0768541134513,"y":241.41674991590497},"p2":{"x":561.4285583496094,"y":259.1428565979004}}},{"id":"dp7088762179086097","type":"rectangle","data":{"p1":{"x":528.0768541134513,"y":278.416749915905},"p2":{"x":561.4285583496094,"y":296.1428565979004}}},{"id":"dp46899738478318853","type":"rectangle","data":{"p1":{"x":580,"y":178.41674991590497},"p2":{"x":630,"y":198.14285278320312}}},{"id":"da5156711271188359","data":[{"x":505.50433907005504,"y":250.13710544533197},{"x":505.4285583496094,"y":287.1428565979004}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da7753207859760989","data":[{"x":505.4285583496094,"y":287.1428565979004},{"x":529.4995021456203,"y":287.2709706669527}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da40898430934028696","data":[{"x":562,"y":250.14285278320312},{"x":597,"y":200.14285278320312}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da75002139300269","data":[{"x":557,"y":126.14285278320312},{"x":595,"y":174.14285278320312}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da06475562154143355","data":[{"p1":{"x":560,"y":306.1428527832031},"p2":{"x":458,"y":330.1428527832031},"cp":{"dx":-14.571441650390625,"dy":46.142852783203125},"cp2":{"dx":29,"dy":16}}],"head":">","tail":"no","shaft":"--","mVer":1,"type":"cubic","style":{"strokeColor":[144,19,254,1]}},{"id":"da690416820412711","data":[{"p1":{"x":613,"y":175.14285278320312},"p2":{"x":507,"y":100.14285278320312},"cp":{"dx":-4,"dy":-37},"cp2":{"dx":78,"dy":-9}}],"head":">","tail":"no","shaft":"--","mVer":1,"type":"cubic","style":{"strokeColor":[144,19,254,1]}}],"settings":{"grid":false,"diagramHeight":405.3333435058594}}]},{"id":"n0.1217711693939072","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":464,"delayRenderCache":{"av":464,"map":{}}}

==> docs/da0d6abe-e0ee-4296-8f82-37d442b143cd <==
{"id":"r0.9651935270262256","lines":[{"id":"n0.2619161131690061","blocks":[]},{"id":"n0.2353290494109901","blocks":[]},{"id":"n0.609049931282583","blocks":[{"id":"n0.3426359148863569","text":"\\diagram","type":"composite","elements":{"de7639749772192224":{"id":"de7639749772192224","lines":[{"id":"n0.8781380894744106","blocks":[{"id":"n0.6924512275307515","text":"r"},{"id":"n0.7238010975500517","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.13649886142583734","lines":[{"id":"n0.20981117247165448","blocks":[{"id":"n0.05068069484039017","text":"t"}]}]}}},{"id":"n0.14741370167325374","text":",s"},{"id":"n0.08134301292273727","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.4143119495011718","lines":[{"id":"n0.0708882123712582","blocks":[{"id":"n0.500714185395958","text":"t"}]}]}}},{"id":"n0.5706095683672192","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9067813294653015","lines":[{"id":"n0.5277801738939238","blocks":[{"id":"n0.3770190964613933","text":"+"}]}]}}},{"id":"n0.6057485771034623","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9858067714391492","lines":[{"id":"n0.6882074882195017","blocks":[{"id":"n0.05517511940550612","text":"1"}]}]}}}]}],"shape":{"data":{"p":{"x":141.45528113942623,"y":310.5244432419479},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"},"style":{"textColor":[245,166,35,1]}},"isMathDisplayMode":true},"de8795771212142249":{"id":"de8795771212142249","lines":[{"id":"n0.667000468794235","blocks":[{"id":"n0.5888477979323106","text":"s"},{"id":"n0.8600433497633744","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5943412513250106","lines":[{"id":"n0.6863009835292035","blocks":[{"id":"n0.16476980076747627","text":"t"}]}]}}}]}],"shape":{"data":{"p":{"x":152.34804794136022,"y":188.73544392061396},"rotation":0},"anchor":"left-top","style":{"textColor":[245,166,35,1]}},"isMathDisplayMode":true},"de5382940630395954":{"id":"de5382940630395954","lines":[{"id":"n0.6501509589970853","blocks":[{"id":"n0.6480187738425032","text":"memory list"}]}],"shape":{"data":{"p":{"x":183.54826110663527,"y":338.09242863950755},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de4336456393056849":{"id":"de4336456393056849","lines":[{"blocks":[{"id":"n0.4444876477139117","text":"Experinece buffer"}],"id":"n0.3215315345450014"}],"shape":{"data":{"p":{"x":253.38737380260147,"y":370.5226416299383},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de8638313643010851":{"id":"de8638313643010851","lines":[{"blocks":[{"id":"n0.7227497685806299","text":"Mini Batch"}],"id":"n0.468084264799451"}],"shape":{"data":{"p":{"x":273.9766460182115,"y":234.43596970123485},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de489851208893364":{"id":"de489851208893364","lines":[{"blocks":[{"text":"Hidden ","id":"n0.08029314994997683"}],"id":"n0.9152362411963197"},{"blocks":[{"text":"Layers","id":"n0.9404929114575815"}],"style":null,"id":"n0.09539425507506283"}],"shape":{"data":{"p":{"x":412.2344691653596,"y":112.53929772874528},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de08634791004831177":{"id":"de08634791004831177","lines":[{"blocks":[{"text":"s","id":"n0.1849559442205173"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"t","id":"n0.6582187836289799"}],"id":"n0.38945112533392945"}],"id":"n0.6454225098861619"}},"id":"n0.6975865629326581"}],"id":"n0.45227860567050504"}],"shape":{"data":{"p":{"x":382.62208266604546,"y":120.95573551950419},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de9037143644634442":{"id":"de9037143644634442","lines":[{"blocks":[{"id":"n0.6527654199580024","text":"Q"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.7150629117744809"}],"id":"n0.8161598537870085"}],"id":"n0.0835933026536102"}},"id":"n0.26663836640897065"}],"id":"n0.9936962503970277"}],"shape":{"data":{"p":{"x":484.61357778485313,"y":99.17175563268465},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\tiny"}},"isMathDisplayMode":true},"de2839329920983895":{"id":"de2839329920983895","lines":[{"blocks":[{"id":"n0.6736936776048337","text":"Prediction Nueral Network"}],"id":"n0.9014661240732309"}],"shape":{"data":{"p":{"x":378.5013851871653,"y":318.4657628563759},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de7748446429291902":{"id":"de7748446429291902","lines":[{"blocks":[{"text":"Target Nueral Network","id":"n0.25243144470676016"}],"id":"n0.39860583496515156"}],"shape":{"data":{"p":{"x":378.4233763229007,"y":178.6806171947381},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de3322389628629139":{"id":"de3322389628629139","lines":[{"blocks":[{"text":"Hidden ","id":"n0.7039114547328817"}],"id":"n0.8807376816154007"},{"blocks":[{"text":"Layers","id":"n0.48525469130423904"}],"style":null,"id":"n0.310673573421153"}],"shape":{"data":{"p":{"x":410.4188673925067,"y":243.99287841717288},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de005188531317795508":{"id":"de005188531317795508","lines":[{"blocks":[{"text":"s","id":"n0.9924230221266865"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"t","id":"n0.4714641376663393"}],"id":"n0.22778988509157871"}],"id":"n0.467609907188991"}},"id":"n0.8632165590563634"}],"id":"n0.06404807538235158"}],"shape":{"data":{"p":{"x":380.80648089319254,"y":252.4093162079318},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de844522307833887":{"id":"de844522307833887","lines":[{"id":"n0.9534840878998827","blocks":[{"id":"n0.8125712056523053","text":"update parameters"}]}],"shape":{"data":{"p":{"x":268.66531348888867,"y":180.00530479704972},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de33724832592648957":{"id":"de33724832592648957","lines":[{"blocks":[{"text":"Q","id":"n0.4588730121106499"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.768964379071412","text":"n"}],"id":"n0.2726560223715051"}],"id":"n0.8854985385960294"}},"id":"n0.8808727815195463"}],"id":"n0.7145265499478859"}],"shape":{"data":{"p":{"x":483.7057768984267,"y":142.68103938167127},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\tiny"}},"isMathDisplayMode":true},"de6196380219930566":{"id":"de6196380219930566","lines":[{"blocks":[{"text":"Q","id":"n0.07755048485160954"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.965182906322624"}],"id":"n0.8562746231443259"}],"id":"n0.3396577214902159"}},"id":"n0.7143456879838277"}],"id":"n0.3733984206671259"}],"shape":{"data":{"p":{"x":481.89017512557376,"y":231.55106576258004},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\tiny"}},"isMathDisplayMode":true},"de9780982456964917":{"id":"de9780982456964917","lines":[{"blocks":[{"text":"Q","id":"n0.927861604965583"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.4430028344181469","text":"n"}],"id":"n0.09278100926377131"}],"id":"n0.6955144934423734"}},"id":"n0.5897048457766239"}],"id":"n0.6575786858622708"}],"shape":{"data":{"p":{"x":481.89017512557376,"y":274.1346200700989},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\tiny"}},"isMathDisplayMode":true},"de1858639352892859":{"id":"de1858639352892859","lines":[{"blocks":[{"id":"n0.7622321965931733","text":"𝜖 greedy"}],"id":"n0.9936555356461236"},{"id":"n0.031097131334195227","blocks":[{"id":"n0.4170993596284924","text":"algorithm"}]}],"shape":{"data":{"p":{"x":544.3838536869557,"y":273.7335403028667},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de5749176392660895":{"id":"de5749176392660895","lines":[{"blocks":[{"id":"n0.36608127889020037","text":"Q"}],"id":"n0.4982026044856065"}],"shape":{"data":{"p":{"x":519.1368204694663,"y":274.8925725474992},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de6432026420400929":{"id":"de6432026420400929","lines":[{"blocks":[{"id":"n0.7718791165284471","text":"      loss "}],"id":"n0.6722203145979655"},{"id":"n0.8340513215097372","blocks":[{"id":"n0.5192740535459104","text":"  Function"}],"style":null}],"shape":{"data":{"p":{"x":541.522152357316,"y":180.374005049526},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de6653291438025923":{"id":"de6653291438025923","lines":[{"blocks":[{"id":"n0.8966955104140477","text":"a"},{"id":"n0.3325773215450598","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.37141218540393695","lines":[{"id":"n0.510462705327412","blocks":[{"id":"n0.5918037924154502","text":"t"}]}]}}}],"id":"n0.37891952887452174"}],"shape":{"data":{"p":{"x":103.28070051754476,"y":149.85480737896634},"rotation":0},"anchor":"left-top","style":{"textColor":[65,117,5,1]}},"isMathDisplayMode":true},"de348733398105175":{"id":"de348733398105175","lines":[{"blocks":[{"id":"n0.24268599099270993","text":"Docking Phase"}],"id":"n0.36835813393698746"},{"id":"n0.6929761653743423","blocks":[{"text":" Envirmoent ","id":"n0.8195573393833739"}],"style":null}],"shape":{"data":{"p":{"x":45.05000974648884,"y":237.34254105542664},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de3943317859587221":{"id":"de3943317859587221","lines":[{"blocks":[{"id":"n0.21383357319062757","text":"Deep Q Learning Architecture"}],"id":"n0.27188326805586116"}],"shape":{"data":{"p":{"x":185.8123043170961,"y":69.23113550094801},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\small"},"style":{"textColor":[20,60,120,1],"strokeType":"--","strokeColor":[20,60,120,1]},"frameType":"rectangle"},"isMathDisplayMode":true},"de13472492480993825":{"id":"de13472492480993825","lines":[{"blocks":[{"text":"DRL Agent ","id":"n0.6628087087913392"}],"id":"n0.6646038765650544"}],"shape":{"data":{"p":{"x":164.05000974648885,"y":11.342541055426636},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\small"},"style":{"textColor":[208,2,27,1]}},"isMathDisplayMode":true},"de5449919228223186":{"id":"de5449919228223186","lines":[{"blocks":[{"id":"n0.957627209025333","text":"Envirmoent"}],"id":"n0.29180138375337417"}],"shape":{"data":{"p":{"x":45.050009746488854,"y":11},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\small"},"style":{"textColor":[208,2,27,1]}},"isMathDisplayMode":true}},"connections":[],"intersections":{"id":"di05442985925027943","items":[],"style":{}},"shapes":[{"id":"dp1589342474521125","type":"image","data":{"p1":{"x":55.86208271048189,"y":174.93189535320764},"p2":{"x":118.94622118388033,"y":238.45659943340962},"url":"data-resources/db02ae9f-e922-4ea2-b522-0a7cd01b9484"}},{"id":"dp10015994215697432","type":"rectangle","data":{"p1":{"x":26.33331298828125,"y":176.5607339193666},"p2":{"x":150.35407700673568,"y":235.19892230109159}},"style":{"thickness":2}},{"id":"dp4641200834783572","type":"ellipse","data":{"p1":{"x":259.6690760325713,"y":285.15306396599124},"p2":{"x":341.65163241217084,"y":315.7752215535497}},"style":{"thickness":2}},{"id":"da3051920589120525","data":[{"x":259.6690760325713,"y":299.64972347669095},{"x":259.6690729604826,"y":350.7952577161856}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"da800652037017791","data":[{"x":341.65163241217084,"y":300.4641427597705},{"x":341.8126958817965,"y":350.7952577161856}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"thickness":2}},{"id":"dp6498600205138614","type":"ellipse","data":{"p1":{"x":259.6690729604826,"y":335.4841789224063},"p2":{"x":341.8126958817965,"y":366.10633650996476}},"style":{"thickness":2}},{"id":"da01568926923172098","data":[{"x":124.33259066256001,"y":234.78362782551088},{"x":124.63723374297248,"y":330.692637140119}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[245,166,35,1]}},{"id":"da5298176720391385","data":[{"x":124.63723374297248,"y":330.692637140119},{"x":203.95970490164768,"y":330.5305035038248}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[245,166,35,1]}},{"id":"da03292121573823592","data":[{"x":154.03065614819252,"y":212.03713499594642},{"x":215.7611164251916,"y":212.03713499594642}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[245,166,35,1]}},{"id":"da06115426673650193","data":[{"x":215.7611164251916,"y":212.03713499594642},{"x":215.7611164251916,"y":326.1663423508993}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[245,166,35,1]}},{"id":"dp854952318315878","type":"rectangle","data":{"p1":{"x":205.44789734352,"y":325.76271796157863},"p2":{"x":228.15819293874944,"y":336.02439347214926}}},{"id":"da8470109036044176","data":[{"x":226.9573227404705,"y":331.1476470477965},{"x":259.93261267219543,"y":331.39574626481027}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[7,144,226,1]}},{"id":"dp38647346813132843","type":"rectangle","data":{"p1":{"x":272.55434983229577,"y":346.2345101969547},"p2":{"x":295.2646454275252,"y":357.3106049906049}}},{"id":"dp8933376951910441","type":"rectangle","data":{"p1":{"x":304.76753529163454,"y":345.4200909138752},"p2":{"x":327.477830886864,"y":356.49618570752534}}},{"id":"dp8055048364268742","type":"rectangle","data":{"p1":{"x":303.9622056551511,"y":320.98751242148984},"p2":{"x":326.6725012503805,"y":332.06360721513994}}},{"id":"dp5104284295487775","type":"rectangle","data":{"p1":{"x":270.9436905593288,"y":320.1730931384103},"p2":{"x":293.6539861545582,"y":331.24918793206047}}},{"id":"dp1304220439242889","type":"rectangle","data":{"p1":{"x":270.1383609228453,"y":296.55493392910444},"p2":{"x":292.8486565180748,"y":307.6310287227546}}},{"id":"dp7572418587488732","type":"rectangle","data":{"p1":{"x":302.35154638218415,"y":296.55493392910444},"p2":{"x":325.06184197741356,"y":307.6310287227546}}},{"id":"da9091903165817103","data":[{"x":300.6603542223711,"y":285.15306396599124},{"x":300.1865988628521,"y":269.740939201691}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"dp2912917223386602","type":"rectangle","data":{"p1":{"x":276.2880246279446,"y":256.24396223432046},"p2":{"x":298.998320223174,"y":267.3200570279706}}},{"id":"dp4748239481122165","type":"rectangle","data":{"p1":{"x":306.89055081431644,"y":256.24396223432046},"p2":{"x":329.6008464095459,"y":267.3200570279706}}},{"id":"dp6032075051564585","type":"rectangle","data":{"p1":{"x":266.624069374154,"y":252.17186581892287},"p2":{"x":339.1037366576663,"y":270.5777341602886}},"style":{"thickness":2}},{"id":"da19354610609573708","data":[{"x":340.65580063886176,"y":261.13047793279753},{"x":381.88867864123324,"y":261.619122046414}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"dp0008165653694707231","type":"ellipse","data":{"p1":{"x":384.6120813005126,"y":126.15798415654274},"p2":{"x":394.80223417118157,"y":136.60853087170216}}},{"id":"dp9789592945089283","type":"ellipse","data":{"p1":{"x":409.35959541499443,"y":69.4483651174231},"p2":{"x":419.54974828566344,"y":79.89891183258251}}},{"id":"dp8297219494129779","type":"ellipse","data":{"p1":{"x":409.35959541499443,"y":170.11178727088182},"p2":{"x":419.54974828566344,"y":180.5623339860412}}},{"id":"dp3616848524594365","type":"ellipse","data":{"p1":{"x":410.08746347718505,"y":85.43156145323502},"p2":{"x":420.277616347854,"y":95.88210816839444}}},{"id":"dp38524805492500747","type":"ellipse","data":{"p1":{"x":410.08746347718505,"y":153.82121467199704},"p2":{"x":420.277616347854,"y":164.27176138715646}}},{"id":"da8269047652009216","data":[{"x":415.1825399125196,"y":95.88210816839444},{"x":415.1825399125196,"y":153.82121467199704}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"dp4539087736568428","type":"ellipse","data":{"p1":{"x":448.66447077328905,"y":69.4483651174231},"p2":{"x":458.854623643958,"y":79.89891183258251}}},{"id":"dp41137669179615033","type":"ellipse","data":{"p1":{"x":448.66447077328905,"y":170.11178727088182},"p2":{"x":458.854623643958,"y":180.5623339860412}}},{"id":"dp07408655413745646","type":"ellipse","data":{"p1":{"x":449.3923388354797,"y":85.43156145323502},"p2":{"x":459.5824917061487,"y":95.88210816839444}}},{"id":"dp15034298494800336","type":"ellipse","data":{"p1":{"x":449.3923388354797,"y":153.82121467199704},"p2":{"x":459.5824917061487,"y":164.27176138715646}}},{"id":"da4656336622873056","data":[{"x":454.4874152708142,"y":95.88210816839444},{"x":454.4874152708142,"y":153.82121467199704}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da7933929685182313","data":[{"x":394.80223417118157,"y":131.38325751412245},{"x":409.35959541499443,"y":74.6736384750028}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9283963821421053","data":[{"x":394.80223417118157,"y":131.38325751412245},{"x":410.8153315393757,"y":94.6526382917198}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6550384168515815","data":[{"x":394.80223417118157,"y":131.38325751412245},{"x":409.35959541499443,"y":175.3370606284615}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da34481025597530834","data":[{"x":394.80223417118157,"y":131.38325751412245},{"x":410.08746347718505,"y":159.04648802957672}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7469749752423971","data":[{"x":419.54974828566344,"y":74.6736384750028},{"x":448.66447077328905,"y":74.6736384750028}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da568370993707602","data":[{"x":419.54974828566344,"y":74.6736384750028},{"x":449.3923388354797,"y":90.65683481081474}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8209209426400641","data":[{"x":420.277616347854,"y":90.65683481081474},{"x":448.66447077328905,"y":74.6736384750028}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da14838008878541742","data":[{"x":420.277616347854,"y":90.65683481081474},{"x":449.3923388354797,"y":90.65683481081474}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da11711322242758371","data":[{"x":419.54974828566344,"y":175.3370606284615},{"x":448.66447077328905,"y":175.3370606284615}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7165505361787865","data":[{"x":420.277616347854,"y":159.04648802957672},{"x":449.3923388354797,"y":159.04648802957672}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9286439750270796","data":[{"x":420.277616347854,"y":159.04648802957672},{"x":448.66447077328905,"y":175.3370606284615}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da3461303721567983","data":[{"x":419.54974828566344,"y":175.3370606284615},{"x":449.3923388354797,"y":159.04648802957672}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp627900848910671","type":"ellipse","data":{"p1":{"x":485.78574194501175,"y":100.9496020198104},"p2":{"x":498.08719210381975,"y":112.32636889881559}}},{"id":"da5883680138742358","data":[{"x":490.8808183803462,"y":112.32636889881559},{"x":490.8808183803462,"y":144.60013783351226}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da413928557893366","data":[{"x":458.854623643958,"y":74.6736384750028},{"x":485.78574194501175,"y":107.10109554123589}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da021379110434450732","data":[{"x":459.5824917061487,"y":90.65683481081474},{"x":485.78574194501175,"y":107.10109554123589}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da1307275658351441","data":[{"x":459.5824917061487,"y":159.04648802957672},{"x":485.78574194501175,"y":149.82541119109197}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da312900120429614","data":[{"x":458.854623643958,"y":175.3370606284615},{"x":485.78574194501175,"y":149.82541119109197}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da11286149279728308","data":[{"p1":{"x":386.42768307336553,"y":234.2546415911736},"p2":{"x":382.1480424076738,"y":154.6419096249428},"cp":{"dx":-30.605866372058983,"dy":-27.771883244033972},"cp2":{"dx":-36.3120354570583,"dy":27.771883244034}}],"head":">","tail":"no","shaft":"-","mVer":1,"type":"cubic","style":{"strokeColor":[20,60,120,1]}},{"id":"dp31466386951367165","type":"ellipse","data":{"p1":{"x":382.7964795276597,"y":257.6115648449703},"p2":{"x":392.98663239832865,"y":268.0621115601298}}},{"id":"dp8882263769238594","type":"ellipse","data":{"p1":{"x":407.5439936421415,"y":200.90194580585072},"p2":{"x":417.7341465128105,"y":211.3524925210101}}},{"id":"dp8057535279850134","type":"ellipse","data":{"p1":{"x":407.5439936421415,"y":301.5653679593094},"p2":{"x":417.7341465128105,"y":312.0159146744688}}},{"id":"dp5034722898936421","type":"ellipse","data":{"p1":{"x":408.27186170433214,"y":216.88514214166264},"p2":{"x":418.4620145750011,"y":227.33568885682206}}},{"id":"dp4109190886802778","type":"ellipse","data":{"p1":{"x":408.27186170433214,"y":285.2747953604246},"p2":{"x":418.4620145750011,"y":295.7253420755841}}},{"id":"da16382607823928463","data":[{"x":413.3669381396667,"y":227.33568885682206},{"x":413.3669381396667,"y":285.2747953604246}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"dp2521080972136902","type":"ellipse","data":{"p1":{"x":446.84886900043614,"y":200.90194580585072},"p2":{"x":457.0390218711051,"y":211.3524925210101}}},{"id":"dp1604328455446027","type":"ellipse","data":{"p1":{"x":446.84886900043614,"y":301.5653679593094},"p2":{"x":457.0390218711051,"y":312.0159146744688}}},{"id":"dp519968262183508","type":"ellipse","data":{"p1":{"x":447.57673706262676,"y":216.88514214166264},"p2":{"x":457.7668899332958,"y":227.33568885682206}}},{"id":"dp7886312482540467","type":"ellipse","data":{"p1":{"x":447.57673706262676,"y":285.2747953604246},"p2":{"x":457.7668899332958,"y":295.7253420755841}}},{"id":"da8620824293727087","data":[{"x":452.6718134979613,"y":227.33568885682206},{"x":452.6718134979613,"y":285.2747953604246}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da09682596363438312","data":[{"x":392.98663239832865,"y":262.8368382025501},{"x":407.5439936421415,"y":206.1272191634304}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5911627203148244","data":[{"x":392.98663239832865,"y":262.8368382025501},{"x":408.99972976652276,"y":226.1062189801474}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6537875126837136","data":[{"x":392.98663239832865,"y":262.8368382025501},{"x":407.5439936421415,"y":306.7906413168891}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6522068488410606","data":[{"x":392.98663239832865,"y":262.8368382025501},{"x":408.27186170433214,"y":290.50006871800434}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9172949695390451","data":[{"x":417.7341465128105,"y":206.1272191634304},{"x":446.84886900043614,"y":206.1272191634304}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9377407711784944","data":[{"x":417.7341465128105,"y":206.1272191634304},{"x":447.57673706262676,"y":222.11041549924232}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9717696765910107","data":[{"x":418.4620145750011,"y":222.11041549924232},{"x":446.84886900043614,"y":206.1272191634304}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da024881965750956914","data":[{"x":418.4620145750011,"y":222.11041549924232},{"x":447.57673706262676,"y":222.11041549924232}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8363564203032521","data":[{"x":417.7341465128105,"y":306.7906413168891},{"x":446.84886900043614,"y":306.7906413168891}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da786590945491642","data":[{"x":418.4620145750011,"y":290.50006871800434},{"x":447.57673706262676,"y":290.50006871800434}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6599152943622968","data":[{"x":418.4620145750011,"y":290.50006871800434},{"x":446.84886900043614,"y":306.7906413168891}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5687040017084417","data":[{"x":417.7341465128105,"y":306.7906413168891},{"x":447.57673706262676,"y":290.50006871800434}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5867162873728369","data":[{"x":489.0652166074933,"y":243.7799495872432},{"x":489.0652166074933,"y":276.05371852193986}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da5277146655649627","data":[{"x":457.0390218711051,"y":206.1272191634304},{"x":483.97014017215884,"y":238.55467622966347}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da704869943367306","data":[{"x":457.7668899332958,"y":222.11041549924232},{"x":483.97014017215884,"y":238.55467622966347}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da0688638849153198","data":[{"x":457.7668899332958,"y":290.50006871800434},{"x":483.97014017215884,"y":281.2789918795196}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da30148004414299256","data":[{"x":457.0390218711051,"y":306.7906413168891},{"x":483.97014017215884,"y":281.2789918795196}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp052583183570326764","type":"ellipse","data":{"p1":{"x":485.78574194501175,"y":144.13702775158936},"p2":{"x":498.08719210381975,"y":155.51379463059456}}},{"id":"dp00618315469967845","type":"ellipse","data":{"p1":{"x":483.97014017215884,"y":232.8662927901609},"p2":{"x":496.27159033096683,"y":244.2430596691661}}},{"id":"dp1485700269367869","type":"ellipse","data":{"p1":{"x":483.97014017215884,"y":275.590608440017},"p2":{"x":496.27159033096683,"y":286.96737531902215}}},{"id":"da19885985323652955","data":[{"x":361.2722396400476,"y":261.3747999896058},{"x":361.0092582534248,"y":351.8222806575842}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da786630486048054","data":[{"x":361.0092582534248,"y":351.8222806575842},{"x":567.9878603586569,"y":350.8965512161164}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da678858238629007","data":[{"x":567.9878603586569,"y":350.8965512161164},{"x":567.9878603586569,"y":302.7586202597908}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"dp5563832997772895","type":"rectangle","data":{"p1":{"x":541.3342253213091,"y":275.9124664572246},"p2":{"x":599.7608913835829,"y":302.7586202597908}}},{"id":"da5834684049276506","data":[{"x":490.8808183803462,"y":128.46325336616394},{"x":521.6900151509076,"y":128.7214852638444}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da16763583332459664","data":[{"x":489.0652166074933,"y":259.9168340545915},{"x":519.8744133780547,"y":260.175065952272}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da2439654120131589","data":[{"x":521.6900151509076,"y":128.7214852638444},{"x":521.6900151509076,"y":186.116710634848}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da6144645077388431","data":[{"x":519.8744133780547,"y":202.7798405812684},{"x":519.8744133780547,"y":260.175065952272}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da1789865030911033","data":[{"x":521.6900151509076,"y":186.116710634848},{"x":545.2928381979955,"y":186.116710634848}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da8210684364264234","data":[{"x":519.8744133780547,"y":202.7798405812684},{"x":543.4772364251426,"y":202.7798405812684}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"dp48382282439863555","type":"rectangle","data":{"p1":{"x":544.0576279805884,"y":181.48806342750902},"p2":{"x":602.4842940428623,"y":208.3342172300752}}},{"id":"da23417042547898648","data":[{"x":519.8744133780547,"y":260.175065952272},{"x":519.8744133780547,"y":290.7241375207094}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da9792324573647748","data":[{"x":519.8744133780547,"y":290.7241375207094},{"x":543.4772364251426,"y":290.7241375207094}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[20,60,120,1]}},{"id":"da8707071167263642","data":[{"x":614.2857055664062,"y":288.8726786377738},{"x":613.3779046799798,"y":38}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[65,117,5,1]}},{"id":"da9945523058230241","data":[{"x":599.7608913835829,"y":288.8726786377738},{"x":614.2857055664062,"y":288.8726786377738}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[65,117,5,1]}},{"id":"da8966548135179726","data":[{"x":613.3779046799798,"y":38},{"x":97.74700118975218,"y":38}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[65,117,5,1]}},{"id":"da50478068860716","data":[{"x":97.74700118975218,"y":38},{"x":97.74700118975218,"y":174.0822278957666}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[65,117,5,1]}},{"id":"dp6643968792592012","type":"rectangle","data":{"p1":{"x":184.89588628669208,"y":63.92041729834327},"p2":{"x":608.1904631278617,"y":386.99999237060547}},"style":{"strokeColor":[20,60,200,1],"boxShadow":{"fill":[0,0,0,0.09]}}},{"id":"da525425600022982","data":[{"x":143,"y":12},{"x":142.28570556640625,"y":176.99999237060547}],"head":"no","tail":"no","shaft":"--","mVer":1,"style":{"thickness":2,"strokeColor":[208,2,27,1]}},{"id":"da10351729005470567","data":[{"x":143,"y":237},{"x":142.28570556640625,"y":401.99999237060547}],"head":"no","tail":"no","shaft":"--","mVer":1,"style":{"thickness":2,"strokeColor":[208,2,27,1]}}],"settings":{"grid":true,"diagramHeight":395.6000061035156}}]},{"id":"n0.7118433622573668","blocks":[],"style":null},{"id":"n0.0013835601885578974","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":1372,"delayRenderCache":{"av":1372,"map":{}}}

==> docs/fd31e4db-564b-4ba5-9c4c-7219c1190ba0 <==
{"id":"r0.9984998352954119","lines":[{"blocks":[{"text":"\\diagram","type":"composite","elements":{"de09089904648312341":{"id":"de09089904648312341","lines":[{"blocks":[{"text":"Hidden ","id":"n0.4648681318928336"}],"id":"n0.9285904482655118"},{"blocks":[{"text":"Layers","id":"n0.8513031314124653"}],"style":null,"id":"n0.9720842598717605"}],"shape":{"data":{"p":{"x":124.85535866057563,"y":190.33480834593192},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de23052219469379964":{"id":"de23052219469379964","lines":[{"blocks":[{"text":"s","id":"n0.8647542393407075"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"t","id":"n0.11884594478422272"}],"id":"n0.9979936004579235"}],"id":"n0.4632811059888533"}},"id":"n0.7843516334870524"}],"id":"n0.8860604723433694"}],"shape":{"data":{"p":{"x":64.13571822830187,"y":202.59195724761253},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de4278195411185204":{"id":"de4278195411185204","lines":[{"id":"n0.6928554778763865","blocks":[{"id":"n0.9025990990149098","text":"|A|"}]}],"shape":{"data":{"p":{"x":389,"y":288.28571701049805}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de06687792709160556":{"id":"de06687792709160556","lines":[{"blocks":[{"id":"n0.6243458676926645","text":"\\sum","type":"composite","elements":{}}],"id":"n0.23552976177126572"}],"shape":{"data":{"p":{"x":411,"y":220.28571701049805}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de1363343582137566":{"id":"de1363343582137566","lines":[{"blocks":[{"text":"\\sum","type":"composite","elements":{},"id":"n0.759818784807134"}],"id":"n0.61146794018223"}],"shape":{"data":{"p":{"x":412,"y":148.28571701049805}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de7361555228289434":{"id":"de7361555228289434","lines":[{"blocks":[{"id":"n0.2788701471877144","text":"V"},{"id":"n0.7542347151280338","type":"single","text":"("},{"id":"n0.17747879583568582","text":"s"},{"id":"n0.7711255500500134","type":"single","text":")"}],"id":"n0.7668221031025879"}],"shape":{"data":{"p":{"x":297,"y":70.28571701049805}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de6108653283384207":{"id":"de6108653283384207","lines":[{"blocks":[{"id":"n0.4545389438577434","text":"A"},{"id":"n0.07433092573329203","type":"single","text":"("},{"id":"n0.7831348303508117","text":"s,a"},{"id":"n0.9646586076821708","type":"single","text":")"}],"id":"n0.38955971005494705"}],"shape":{"data":{"p":{"x":293,"y":208.28571701049805}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de9835469962524281":{"id":"de9835469962524281","lines":[{"blocks":[{"id":"n0.9690487700358088","text":"Q"},{"id":"n0.24295271799894835","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.13477248814862786","lines":[{"id":"n0.26844851302179484","blocks":[{"id":"n0.8733079162768376","text":"1"}]}]}}}],"id":"n0.0216650916809773"}],"shape":{"data":{"p":{"x":459,"y":116.28571701049805}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de8024028799571241":{"id":"de8024028799571241","lines":[{"blocks":[{"text":"Q","id":"n0.008609513016125891"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.3938561700129799","text":"n"}],"id":"n0.3309901245417959"}],"id":"n0.5113034479472245"}},"id":"n0.26281687784515473"}],"id":"n0.7265193427716059"}],"shape":{"data":{"p":{"x":459,"y":200.28571701049805}},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de10697832361774129":{"id":"de10697832361774129","lines":[{"id":"n0.2879727489789501","blocks":[{"id":"n0.7129429037898238","text":"Q"},{"id":"n0.5342091273172858","type":"single","text":"("},{"id":"n0.6287052919095732","text":"s,a"},{"id":"n0.9803155447765122","type":"single","text":")"},{"id":"n0.6041838502337677","text":"=V"},{"id":"n0.3411969216843258","type":"single","text":"("},{"id":"n0.7563805818669376","text":"s"},{"id":"n0.12205237929615209","type":"single","text":")"},{"id":"n0.4515025290774961","text":"+"},{"id":"n0.49761936977004506","type":"single","text":"("},{"id":"n0.9251919760915588","text":"A"},{"id":"n0.07245098588688692","type":"single","text":"("},{"id":"n0.6371640465319655","text":"s,a"},{"id":"n0.37568180045953103","type":"single","text":")"},{"id":"n0.7258095959675863","text":"-"},{"id":"n0.6100121024973837","text":"\\frac","type":"composite","elements":{"value":{"id":"n0.8777100078178304","lines":[{"id":"n0.6243297920090576","blocks":[{"id":"n0.9325550463371632","text":"1"}]}]},"sub1":{"id":"n0.622780308147767","lines":[{"id":"n0.7146738424458552","blocks":[{"id":"n0.6404026379667369","text":"|A|"}]}]}}},{"id":"n0.049666134435730314","text":"\\sum","type":"composite","elements":{"from":{"id":"n0.01429332364620306","lines":[{"id":"n0.9376700631295276","blocks":[]}]},"to":{"id":"n0.8518046334724596","lines":[{"id":"n0.47996238658787793","blocks":[{"id":"n0.39621198192487417","text":"a"}]}]}}},{"id":"n0.45640201785341716","text":"A"},{"id":"n0.3939636523287058","type":"single","text":"("},{"id":"n0.35079527459997517","text":"s,a"},{"id":"n0.41287365147104294","type":"single","text":")"},{"id":"n0.7539196772884802","type":"single","text":")"}]}],"shape":{"data":{"p":{"x":364,"y":48}},"anchor":"left-top","style":{"textColor":[208,2,27,1]}},"isMathDisplayMode":true},"de16639299310394828":{"id":"de16639299310394828","lines":[{"id":"n0.22914678849037018","blocks":[{"id":"n0.5136886129880034","text":"     Duleing  DQN Architecture of"}]},{"id":"n0.663355530478545","blocks":[{"id":"n0.7643033955874854","text":"Targer & Prediction Nueral Networks"}],"style":null}],"shape":{"data":{"p":{"x":161,"y":4}},"anchor":"left-top","style":{"textColor":[20,60,120,1]}},"isMathDisplayMode":true},"de8586840866561116":{"id":"de8586840866561116","lines":[{"blocks":[{"id":"n0.8924061934415992","text":"Output"}],"id":"n0.6878389224111592"},{"id":"n0.2129629286086101","blocks":[{"text":" Layer","id":"n0.4016894744348074"}],"style":null}],"shape":{"data":{"p":{"x":247.85535866057563,"y":91.33480834593192},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true},"de186180835340233":{"id":"de186180835340233","lines":[{"blocks":[{"text":"Output","id":"n0.8087061875981738"}],"id":"n0.48419813350773144"},{"blocks":[{"text":" Layer","id":"n0.8863940192133783"}],"style":null,"id":"n0.3717522352048117"}],"shape":{"data":{"p":{"x":271.85535866057563,"y":303.33480834593195},"rotation":0},"anchor":"left-top","settings":{"fontSize":"\\scriptsize"}},"isMathDisplayMode":true}},"connections":[],"intersections":{"id":"di05442985925027943","items":[],"style":{}},"shapes":[{"id":"dp6706860270311694","type":"ellipse","data":{"p1":{"x":61.83898427091685,"y":202.62676282746915},"p2":{"x":79.2974317341911,"y":223.11491031764925}}},{"id":"dp9848885896102013","type":"ellipse","data":{"p1":{"x":104.23807096744008,"y":91.4483651174231},"p2":{"x":121.69651843071443,"y":111.9365126076032}}},{"id":"dp5734034503566838","type":"ellipse","data":{"p1":{"x":104.23807096744008,"y":288.79756570562074},"p2":{"x":121.69651843071443,"y":309.2857131958008}}},{"id":"dp7434103268809471","type":"ellipse","data":{"p1":{"x":105.48510292910254,"y":122.78319312384721},"p2":{"x":122.94355039237672,"y":143.27134061402734}}},{"id":"dp25271845328395437","type":"ellipse","data":{"p1":{"x":105.48510292910254,"y":256.8601309280425},"p2":{"x":122.94355039237672,"y":277.34827841822266}}},{"id":"da9263229960306669","data":[{"x":114.21432666073974,"y":143.27134061402734},{"x":114.21432666073974,"y":256.8601309280425}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"dp7933335781673834","type":"ellipse","data":{"p1":{"x":171.5777968972123,"y":91.4483651174231},"p2":{"x":189.03624436048653,"y":111.9365126076032}}},{"id":"dp10071685909667405","type":"ellipse","data":{"p1":{"x":171.5777968972123,"y":288.79756570562074},"p2":{"x":189.03624436048653,"y":309.2857131958008}}},{"id":"dp760311611223855","type":"ellipse","data":{"p1":{"x":172.8248288588747,"y":122.78319312384721},"p2":{"x":190.28327632214905,"y":143.27134061402734}}},{"id":"dp7351272587447757","type":"ellipse","data":{"p1":{"x":172.8248288588747,"y":256.8601309280425},"p2":{"x":190.28327632214905,"y":277.34827841822266}}},{"id":"da009114323547545933","data":[{"x":181.5540525905119,"y":143.27134061402734},{"x":181.5540525905119,"y":256.8601309280425}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da6887205905145286","data":[{"x":79.2974317341911,"y":212.8708365725592},{"x":104.23807096744008,"y":101.69243886251314}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da0769681491344194","data":[{"x":79.2974317341911,"y":212.8708365725592},{"x":106.73213489076494,"y":140.86098249070503}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da059403023126904264","data":[{"x":79.2974317341911,"y":212.8708365725592},{"x":104.23807096744008,"y":299.0416394507107}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da16708841467225133","data":[{"x":79.2974317341911,"y":212.8708365725592},{"x":105.48510292910254,"y":267.10420467313253}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da017528668772850864","data":[{"x":121.69651843071443,"y":101.69243886251314},{"x":171.5777968972123,"y":101.69243886251314}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da07433977617885312","data":[{"x":121.69651843071443,"y":101.69243886251314},{"x":172.8248288588747,"y":133.02726686893732}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da3144469591875281","data":[{"x":122.94355039237672,"y":133.02726686893732},{"x":171.5777968972123,"y":101.69243886251314}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8047366801100555","data":[{"x":122.94355039237672,"y":133.02726686893732},{"x":172.8248288588747,"y":133.02726686893732}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7737502271348842","data":[{"x":121.69651843071443,"y":299.0416394507107},{"x":171.5777968972123,"y":299.0416394507107}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da11051310057125163","data":[{"x":122.94355039237672,"y":267.10420467313253},{"x":172.8248288588747,"y":267.10420467313253}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da684181148872052","data":[{"x":122.94355039237672,"y":267.10420467313253},{"x":171.5777968972123,"y":299.0416394507107}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da47061583916177185","data":[{"x":121.69651843071443,"y":299.0416394507107},{"x":172.8248288588747,"y":267.10420467313253}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp6119406576989828","type":"ellipse","data":{"p1":{"x":239.17642694199708,"y":213.2060898920518},"p2":{"x":260.25208930402187,"y":235.51007877718246}}},{"id":"da7492717928295745","data":[{"x":247.90565067363423,"y":235.51007877718246},{"x":247.90565067363423,"y":298.7823415611847}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da01674975789823896","data":[{"x":189.03624436048653,"y":101.69243886251314},{"x":238.17642694199708,"y":60.35808433461713}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da9492876867828501","data":[{"x":190.28327632214905,"y":133.02726686893732},{"x":238.17642694199708,"y":60.35808433461713}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp4264831960540332","type":"ellipse","data":{"p1":{"x":239.17642694199708,"y":297.8744208637094},"p2":{"x":260.25208930402187,"y":320.17840974884007}}},{"id":"dp4448891876809371","type":"ellipse","data":{"p1":{"x":238.17642694199708,"y":49.20608989205181},"p2":{"x":259.25208930402187,"y":71.51007877718246}}},{"id":"da6683455178709754","data":[{"x":246.90565067363423,"y":71.51007877718246},{"x":246.90565067363423,"y":134.7823415611847}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"dp310179303217329","type":"ellipse","data":{"p1":{"x":238.17642694199708,"y":133.87442086370942},"p2":{"x":259.25208930402187,"y":156.17840974884007}}},{"id":"da057492993987811714","data":[{"x":189.03624436048653,"y":101.69243886251314},{"x":238.17642694199708,"y":145.02641530627474}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5059134792427213","data":[{"x":190.28327632214905,"y":133.02726686893732},{"x":238.17642694199708,"y":145.02641530627474}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp340439750000175","type":"ellipse","data":{"p1":{"x":299.1764269419971,"y":90.87442086370942},"p2":{"x":320.25208930402187,"y":113.17840974884007}}},{"id":"da4011946302583773","data":[{"x":299.1764269419971,"y":102.02641530627474},{"x":259.25208930402187,"y":60.35808433461713}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6732458327247415","data":[{"x":259.25208930402187,"y":145.02641530627474},{"x":299.1764269419971,"y":102.02641530627474}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da42885104050631506","data":[{"x":190.28327632214905,"y":267.1042046731326},{"x":239.17642694199708,"y":224.35808433461713}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6519541027686389","data":[{"x":190.28327632214905,"y":267.1042046731326},{"x":239.17642694199708,"y":309.02641530627477}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da6944685990821893","data":[{"x":189.03624436048653,"y":299.04163945071076},{"x":239.17642694199708,"y":224.35808433461713}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da10418330218252736","data":[{"x":189.03624436048653,"y":299.04163945071076},{"x":239.17642694199708,"y":309.02641530627477}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp9552673961165732","type":"ellipse","data":{"p1":{"x":301.1764269419971,"y":228.87442086370942},"p2":{"x":322.25208930402187,"y":251.17840974884007}}},{"id":"dp9900451372406167","type":"ellipse","data":{"p1":{"x":302.1764269419971,"y":276.8744208637094},"p2":{"x":323.25208930402187,"y":299.17840974884007}}},{"id":"da9064742689790097","data":[{"x":260.25208930402187,"y":224.35808433461713},{"x":301.1764269419971,"y":240.02641530627474}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da8583319678138461","data":[{"x":260.25208930402187,"y":309.02641530627477},{"x":301.1764269419971,"y":240.02641530627474}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da7990344377056697","data":[{"x":260.25208930402187,"y":309.02641530627477},{"x":302.1764269419971,"y":288.02641530627477}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da29306636108165085","data":[{"x":260.25208930402187,"y":224.35808433461713},{"x":302.1764269419971,"y":288.02641530627477}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da431920033527436","data":[{"x":311.7142581230095,"y":251.17840974884007},{"x":312.7142581230095,"y":276.8744208637095}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da4060933115569516","data":[{"x":327.4285583496094,"y":266.57142639160156},{"x":363.4285583496094,"y":266.57142639160156}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da9239867637652874","data":[{"x":363.4285583496094,"y":236.57142639160156},{"x":363.4285583496094,"y":266.57142639160156}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da5766977132065361","data":[{"x":363.4285583496094,"y":236.57142639160156},{"x":410.4285583496094,"y":237.57142639160156}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da7897687707283598","data":[{"x":363.4285583496094,"y":266.57142639160156},{"x":363.4285583496094,"y":296.57142639160156}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"da06944923076255471","data":[{"x":363.4285583496094,"y":296.57142639160156},{"x":389.4285583496094,"y":297.57142639160156}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"dp315317718905175","type":"ellipse","data":{"p1":{"x":389.85711669921875,"y":285.7051413301397},"p2":{"x":410.93277906124354,"y":308.0091302152704}}},{"id":"da941159918388444","data":[{"x":421.4285583496094,"y":296.57142639160156},{"x":421.4285583496094,"y":246.57142639160156}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da9572657325005316","data":[{"x":410.93277906124354,"y":296.8571357727051},{"x":421.4285583496094,"y":296.57142639160156}],"head":"no","tail":"no","shaft":"-","mVer":1},{"id":"dp9520888781823427","type":"ellipse","data":{"p1":{"x":410.4285583496094,"y":226.41943194903624},"p2":{"x":431.50422071163416,"y":248.7234208341669}}},{"id":"da5657767973838117","data":[{"x":420.96638953062177,"y":226.41943194903624},{"x":420.96638953062177,"y":176.41943194903624}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"dp31634544514915075","type":"ellipse","data":{"p1":{"x":411.4285583496094,"y":154.41943194903624},"p2":{"x":432.50422071163416,"y":176.72342083416686}}},{"id":"da37837731587882706","data":[{"x":320.25208930402187,"y":102.02641530627474},{"x":411.4285583496094,"y":165.57142639160156}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da9339554519714348","data":[{"x":432.50422071163416,"y":165.57142639160156},{"x":458.4285583496094,"y":166.57142639160156}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"dp6218444921166073","type":"ellipse","data":{"p1":{"x":457.1764269419971,"y":114.2060898920518},"p2":{"x":478.25208930402187,"y":136.51007877718246}}},{"id":"dp6806351259291084","type":"ellipse","data":{"p1":{"x":457.1764269419971,"y":198.87442086370942},"p2":{"x":478.25208930402187,"y":221.17840974884007}}},{"id":"da075106227989435","data":[{"x":467.7142581230095,"y":135.60215807970718},{"x":467.7142581230095,"y":198.87442086370942}],"head":"no","tail":"no","shaft":".","mVer":1}],"settings":{"grid":false,"diagramHeight":338.9270935058594,"gridBold":false},"id":"n0.5371754682063783"}],"id":"n0.1756090148386682"}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":363,"delayRenderCache":{"av":363,"map":{}}}

==> resources/b663c298-b148-4425-918a-23e2f39d533f <==
<?xml version="1.0" encoding="UTF-8" standalone="no"?>
<svg
   xmlns:dc="http://purl.org/dc/elements/1.1/"
   xmlns:cc="http://creativecommons.org/ns#"
   xmlns:rdf="http://www.w3.org/1999/02/22-rdf-syntax-ns#"
   xmlns:svg="http://www.w3.org/2000/svg"
   xmlns="http://www.w3.org/2000/svg"
   xmlns:sodipodi="http://sodipodi.sourceforge.net/DTD/sodipodi-0.dtd"
   xmlns:inkscape="http://www.inkscape.org/namespaces/inkscape"
   version="1.1"
   id="svg2"
   viewBox="0 0 2048 1448"
   height="1448"
   width="2048"
   inkscape:version="0.91 r13725"
   sodipodi:docname="quadcopter_icon_03.s.svg"
   inkscape:export-filename="V:\Kunst\Grafik\Commons\Icons\aerial\quadcopter_icon_03.s.png"
   inkscape:export-xdpi="180"
   inkscape:export-ydpi="180">
  <sodipodi:namedview
     pagecolor="#ffffff"
     bordercolor="#666666"
     borderopacity="1"
     objecttolerance="10"
     gridtolerance="10"
     guidetolerance="10"
     inkscape:pageopacity="0"
     inkscape:pageshadow="2"
     inkscape:window-width="640"
     inkscape:window-height="480"
     id="namedview7"
     showgrid="false"
     inkscape:zoom="0.23046875"
     inkscape:cx="1085.3277"
     inkscape:cy="884.03398"
     inkscape:current-layer="svg2" />
  <defs
     id="defs4" />
  <metadata
     id="metadata7">
    <rdf:RDF>
      <cc:Work
         rdf:about="">
        <dc:format>image/svg+xml</dc:format>
        <dc:type
           rdf:resource="http://purl.org/dc/dcmitype/StillImage" />
        <dc:title></dc:title>
      </cc:Work>
    </rdf:RDF>
  </metadata>
  <g
     style="display:inline;opacity:1"
     transform="translate(0,-5549.4995)"
     id="g4353">
    <path
       transform="translate(0,5208.6928)"
       id="ellipse4357"
       d="M 405.60938,550.16797 C 185.03119,551.22788 19.864161,627.3075 8.9824219,733.81445 2.818598,794.13766 47.447704,857.15348 133.05078,909 c 85.60308,51.84651 205.16794,88.27668 332.39258,101.2754 56.36221,5.6604 112.7285,6.5649 166.51367,2.6719 -32.77984,-14.85942 -69.11979,-30.16277 -109.21484,-46.49027 -15.87341,-0.58035 -31.82125,-1.65682 -47.74414,-3.22265 -204.372,-20.88095 -362.0225,-116.363 -352.12305,-213.26563 8.52755,-83.46597 139.88267,-142.70891 314.10156,-141.66406 24.43605,0.14648 49.18438,1.49107 73.875,4.01367 204.37367,20.88106 362.02483,116.36439 352.12305,213.26758 -4.03509,38.54305 -34.73652,73.262 -87.35938,98.79101 32.23922,10.0023 64.77575,18.77203 98.45118,25.58203 56.75546,-31.9869 89.58033,-73.09734 94.31445,-118.12109 C 974.54468,771.51468 929.91558,708.49885 844.3125,656.65234 758.70942,604.80583 639.14455,568.37565 511.91992,555.37695 c -32.00693,-3.27014 -64.08868,-5.0132 -95.76562,-5.20312 -3.52877,-0.0212 -7.04369,-0.0227 -10.54492,-0.006 z m 1236.78122,0 c -3.5012,-0.0168 -7.0161,-0.0153 -10.5449,0.006 -31.6769,0.18992 -63.7587,1.93298 -95.7656,5.20312 -127.2246,12.99869 -246.7895,49.42888 -332.3926,101.27539 -85.6031,51.84651 -130.2322,114.86234 -124.0684,175.18555 4.679,45.02709 37.448,86.14892 94.1543,118.1543 33.7954,-6.8272 66.4436,-15.63028 98.793,-25.67188 -52.6713,-25.50291 -83.4364,-60.20245 -87.541,-98.73633 -9.8994,-96.90261 147.751,-192.38466 352.123,-213.26562 24.6906,-2.5226 49.4389,-3.86719 73.875,-4.01367 174.2189,-1.04485 305.574,58.19809 314.1016,141.66406 9.8995,96.90262 -147.751,192.38467 -352.123,213.26563 -15.8943,1.55177 -31.812,2.61582 -47.6543,3.18554 -40.2232,16.3791 -76.6673,31.728 -109.5313,46.63084 53.868,3.8701 110.3131,2.9306 166.7402,-2.7754 C 1709.7812,997.27669 1829.3461,960.84652 1914.9492,909 2000.5523,857.15349 2045.1814,794.13767 2039.0176,733.81445 2028.1358,627.30749 1862.9688,551.22788 1642.3906,550.16797 Z M 496.16211,817.32422 c -21.39379,-0.13801 -42.63912,1.62891 -46.32813,5.22656 -9.94726,9.7008 -11.33398,32.71466 -11.33398,45.03516 0,18.81126 14.81563,34.9117 35.82422,41.59765 l -0.0918,0.0332 c 178.08765,70.9248 294.10114,119.91301 371.60742,194.76561 -37.97645,53.7335 -106.30592,86.5126 -181.01562,119.3028 -1.03169,-2.7351 -2.44394,-5.1731 -4.41016,-7.0215 -6.02537,-5.6643 -60.63431,-5.7525 -65.82617,-0.6895 -6.99958,6.8262 -7.97461,23.0199 -7.97461,31.6895 0,17.4536 18.11567,31.6035 40.46289,31.6035 8.48075,0 16.34846,-2.0407 22.85156,-5.5234 73.30006,-28.7837 151.52507,-64.26 271.25977,-77.5665 l 0,-3.0918 c 0.002,-20.3387 19.12446,-34.594 31.56026,-44.1496 l 10.01954,-7.6989 0,51.8485 -9.21597,0 0,50.877 148.60097,0 c 25.2496,0 49.4977,18.3928 61.1778,33.0078 11.68,14.6148 21.9097,33.8111 22.2441,54.1699 l 0.7715,46.916 -4.4707,-14.0507 -24.0508,0 0,16.7773 c -22.0508,-55.0029 -75.3353,-91.0677 -134.5937,-91.0976 -80.12875,0 -145.08594,64.9572 -145.08597,145.0859 3e-5,80.1287 64.95722,145.0859 145.08597,145.0859 59.2888,-0.05 112.5819,-36.1694 134.5937,-91.2207 l 0,10.4239 24.0508,0 6.4746,-23.125 0,-3.0157 26.8965,-0.055 3.5351,-23.8964 -2.164,-120.7969 c -0.7871,-39.7102 -8.7191,-66.9314 -27.5762,-89.6777 -21.8149,-26.3144 -75.9882,-44.977 -103.7737,-45.3887 l 0,-52.1884 33.2073,16.536 c 36.1492,4.8545 69.8187,24.368 95.4082,53.4414 73.7355,16.928 130.3073,41.6911 184.1895,62.8497 6.5031,3.4825 14.3708,5.5234 22.8515,5.5234 22.3472,0 40.4629,-14.1499 40.4629,-31.6035 0,-8.6696 -0.975,-24.8633 -7.9746,-31.6895 -5.1918,-5.063 -59.8009,-4.9748 -65.8262,0.6895 -1.9662,1.8484 -3.3784,4.2864 -4.4101,7.0215 -74.7102,-32.7904 -143.039,-65.569 -181.0156,-119.3028 77.5063,-74.8526 193.5198,-123.84081 371.6074,-194.76561 l -0.092,-0.0332 c 21.0086,-6.68595 35.8242,-22.78639 35.8242,-41.59765 0,-12.3205 -1.3867,-35.33436 -11.334,-45.03516 -7.378,-7.1953 -84.9844,-7.06893 -93.5469,0.98047 -10.5333,9.9021 -10.125,31.51239 -10.125,44.05469 0,5.17928 1.1377,10.14792 3.2032,14.77734 -156.5149,53.43022 -288.9602,117.67582 -472.0625,117.67582 l -3.2696,0 c -183.10219,0 -315.54757,-64.2456 -472.06247,-117.67582 2.06544,-4.62942 3.20313,-9.59806 3.20313,-14.77734 0,-12.5423 0.40833,-34.15259 -10.125,-44.05469 -4.28127,-4.0247 -25.82496,-6.06902 -47.21875,-6.20703 z m 82.92578,240.33788 c -173.44528,-0.1323 -305.9272,46.5863 -309.40039,110.4082 -3.8534,70.8394 151.86466,136.9088 347.80664,147.5703 127.9877,6.8732 247.27619,-11.714 312.16602,-48.6406 -5.46184,-6.5906 -8.45766,-14.8778 -8.47266,-23.4375 l 0,-12.6504 c -11.91643,1.3673 -23.41097,2.9501 -34.48047,4.7441 -29.85813,28.8986 -97.94892,48.9755 -183.1543,54.004 -13.16604,5.2368 -26.1599,10.4791 -39.1582,15.5957 -11.33353,5.6514 -24.03269,8.6093 -37.31836,8.6093 -18.56075,0 -36.02775,-5.6386 -50.15625,-16.6738 -4.53804,-3.5445 -8.76524,-7.8209 -12.42187,-12.6738 -128.19115,-16.6082 -218.34973,-62.5862 -215.91407,-110.1094 2.80115,-51.4933 113.0483,-88.7421 255.04688,-86.1719 9.21785,0.167 18.46704,0.5027 27.71289,1.0059 56.02387,3.0872 110.36755,12.2356 155.87305,26.2402 3.23218,-2.6925 6.33699,-5.4232 9.29492,-8.2012 -14.90597,-11.9797 -31.36978,-23.4434 -49.50391,-34.664 -37.01445,-6.7444 -76.06948,-11.3104 -115.55469,-13.5098 -11.82896,-0.6432 -23.6621,-1.0721 -35.45507,-1.2851 -5.67731,-0.1028 -11.31515,-0.1559 -16.91016,-0.1602 z m 885.41601,0.014 c -4.1595,0.022 -8.3273,0.069 -12.5019,0.1445 -11.7931,0.2137 -23.6262,0.6433 -35.4551,1.2871 -39.4769,2.1963 -78.5252,6.7584 -115.5352,13.4981 -18.1418,11.2244 -34.6121,22.6916 -49.5234,34.6757 2.9248,2.7469 5.9924,5.4481 9.1855,8.1114 45.5666,-13.9813 99.949,-23.0985 155.9824,-26.1504 9.246,-0.5032 18.495,-0.8389 27.7129,-1.0059 141.9986,-2.5702 252.2458,34.6786 255.0469,86.1719 2.5649,47.5642 -87.663,93.6058 -215.9922,110.2168 -3.6383,4.8093 -7.8387,9.0477 -12.3437,12.5664 -14.1285,11.0352 -31.5955,16.6738 -50.1563,16.6738 -13.2856,0 -25.9848,-2.9579 -37.3183,-8.6093 -13.0945,-5.1545 -26.1825,-10.4375 -39.4493,-15.7129 -35.3933,-2.0967 -68.3563,-6.8297 -96.9589,-13.9219 2.5201,10.3096 4.2291,21.1111 5.2246,32.3574 54.4435,8.3541 115.859,10.9965 178.084,7.6621 195.942,-10.6615 351.66,-76.7309 347.8066,-147.5703 -3.3939,-62.4283 -130.6163,-109.0264 -301.3574,-110.3789 -4.1405,-0.033 -8.2917,-0.037 -12.4512,-0.016 z m -441.2734,253.7168 c 67.9194,-5e-4 122.979,55.0591 122.9785,122.9785 -6e-4,67.9186 -55.0599,122.9771 -122.9785,122.9766 -67.91786,-6e-4 -122.97603,-55.0587 -122.97659,-122.9766 -4.9e-4,-67.9186 55.05798,-122.9779 122.97659,-122.9785 z m 0,24.832 c -54.20437,3e-4 -98.14531,43.9421 -98.14456,98.1465 3.5e-4,54.2036 43.94097,98.1442 98.14456,98.1445 54.2036,-4e-4 98.1441,-43.9409 98.1445,-98.1445 8e-4,-54.2043 -43.9402,-98.1461 -98.1445,-98.1465 z m -1.6739,7.5899 c 21.3193,0.1392 40.4446,9.3561 50.3067,26.5136 16.2883,28.3378 -20.6126,28.455 -55.5879,48.5586 -34.97532,20.1038 -54.78196,52.5819 -71.07032,24.2442 -16.28834,-28.3377 -1.13932,-67.6074 33.83594,-87.711 13.11572,-7.5388 27.15798,-11.3127 40.44528,-11.5898 0.6921,-0.014 1.3826,-0.02 2.0703,-0.016 z"
       style="color:#000000;display:inline;overflow:visible;visibility:visible;opacity:1;fill:#000000;fill-opacity:1;fill-rule:nonzero;stroke:none;stroke-width:8;stroke-linecap:round;stroke-linejoin:round;stroke-miterlimit:4;stroke-dasharray:none;stroke-dashoffset:0;stroke-opacity:0.59607843;marker:none;enable-background:accumulate"
       inkscape:connector-curvature="0" />
  </g>
</svg>


==> resources/db02ae9f-e922-4ea2-b522-0a7cd01b9484 <==
<?xml version="1.0" encoding="UTF-8" standalone="no"?>
<svg
   xmlns:dc="http://purl.org/dc/elements/1.1/"
   xmlns:cc="http://creativecommons.org/ns#"
   xmlns:rdf="http://www.w3.org/1999/02/22-rdf-syntax-ns#"
   xmlns:svg="http://www.w3.org/2000/svg"
   xmlns="http://www.w3.org/2000/svg"
   xmlns:sodipodi="http://sodipodi.sourceforge.net/DTD/sodipodi-0.dtd"
   xmlns:inkscape="http://www.inkscape.org/namespaces/inkscape"
   version="1.1"
   id="svg2"
   viewBox="0 0 2048 1448"
   height="1448"
   width="2048"
   inkscape:version="0.91 r13725"
   sodipodi:docname="quadcopter_icon_03.s.svg"
   inkscape:export-filename="V:\Kunst\Grafik\Commons\Icons\aerial\quadcopter_icon_03.s.png"
   inkscape:export-xdpi="180"
   inkscape:export-ydpi="180">
  <sodipodi:namedview
     pagecolor="#ffffff"
     bordercolor="#666666"
     borderopacity="1"
     objecttolerance="10"
     gridtolerance="10"
     guidetolerance="10"
     inkscape:pageopacity="0"
     inkscape:pageshadow="2"
     inkscape:window-width="640"
     inkscape:window-height="480"
     id="namedview7"
     showgrid="false"
     inkscape:zoom="0.23046875"
     inkscape:cx="1085.3277"
     inkscape:cy="884.03398"
     inkscape:current-layer="svg2" />
  <defs
     id="defs4" />
  <metadata
     id="metadata7">
    <rdf:RDF>
      <cc:Work
         rdf:about="">
        <dc:format>image/svg+xml</dc:format>
        <dc:type
           rdf:resource="http://purl.org/dc/dcmitype/StillImage" />
        <dc:title></dc:title>
      </cc:Work>
    </rdf:RDF>
  </metadata>
  <g
     style="display:inline;opacity:1"
     transform="translate(0,-5549.4995)"
     id="g4353">
    <path
       transform="translate(0,5208.6928)"
       id="ellipse4357"
       d="M 405.60938,550.16797 C 185.03119,551.22788 19.864161,627.3075 8.9824219,733.81445 2.818598,794.13766 47.447704,857.15348 133.05078,909 c 85.60308,51.84651 205.16794,88.27668 332.39258,101.2754 56.36221,5.6604 112.7285,6.5649 166.51367,2.6719 -32.77984,-14.85942 -69.11979,-30.16277 -109.21484,-46.49027 -15.87341,-0.58035 -31.82125,-1.65682 -47.74414,-3.22265 -204.372,-20.88095 -362.0225,-116.363 -352.12305,-213.26563 8.52755,-83.46597 139.88267,-142.70891 314.10156,-141.66406 24.43605,0.14648 49.18438,1.49107 73.875,4.01367 204.37367,20.88106 362.02483,116.36439 352.12305,213.26758 -4.03509,38.54305 -34.73652,73.262 -87.35938,98.79101 32.23922,10.0023 64.77575,18.77203 98.45118,25.58203 56.75546,-31.9869 89.58033,-73.09734 94.31445,-118.12109 C 974.54468,771.51468 929.91558,708.49885 844.3125,656.65234 758.70942,604.80583 639.14455,568.37565 511.91992,555.37695 c -32.00693,-3.27014 -64.08868,-5.0132 -95.76562,-5.20312 -3.52877,-0.0212 -7.04369,-0.0227 -10.54492,-0.006 z m 1236.78122,0 c -3.5012,-0.0168 -7.0161,-0.0153 -10.5449,0.006 -31.6769,0.18992 -63.7587,1.93298 -95.7656,5.20312 -127.2246,12.99869 -246.7895,49.42888 -332.3926,101.27539 -85.6031,51.84651 -130.2322,114.86234 -124.0684,175.18555 4.679,45.02709 37.448,86.14892 94.1543,118.1543 33.7954,-6.8272 66.4436,-15.63028 98.793,-25.67188 -52.6713,-25.50291 -83.4364,-60.20245 -87.541,-98.73633 -9.8994,-96.90261 147.751,-192.38466 352.123,-213.26562 24.6906,-2.5226 49.4389,-3.86719 73.875,-4.01367 174.2189,-1.04485 305.574,58.19809 314.1016,141.66406 9.8995,96.90262 -147.751,192.38467 -352.123,213.26563 -15.8943,1.55177 -31.812,2.61582 -47.6543,3.18554 -40.2232,16.3791 -76.6673,31.728 -109.5313,46.63084 53.868,3.8701 110.3131,2.9306 166.7402,-2.7754 C 1709.7812,997.27669 1829.3461,960.84652 1914.9492,909 2000.5523,857.15349 2045.1814,794.13767 2039.0176,733.81445 2028.1358,627.30749 1862.9688,551.22788 1642.3906,550.16797 Z M 496.16211,817.32422 c -21.39379,-0.13801 -42.63912,1.62891 -46.32813,5.22656 -9.94726,9.7008 -11.33398,32.71466 -11.33398,45.03516 0,18.81126 14.81563,34.9117 35.82422,41.59765 l -0.0918,0.0332 c 178.08765,70.9248 294.10114,119.91301 371.60742,194.76561 -37.97645,53.7335 -106.30592,86.5126 -181.01562,119.3028 -1.03169,-2.7351 -2.44394,-5.1731 -4.41016,-7.0215 -6.02537,-5.6643 -60.63431,-5.7525 -65.82617,-0.6895 -6.99958,6.8262 -7.97461,23.0199 -7.97461,31.6895 0,17.4536 18.11567,31.6035 40.46289,31.6035 8.48075,0 16.34846,-2.0407 22.85156,-5.5234 73.30006,-28.7837 151.52507,-64.26 271.25977,-77.5665 l 0,-3.0918 c 0.002,-20.3387 19.12446,-34.594 31.56026,-44.1496 l 10.01954,-7.6989 0,51.8485 -9.21597,0 0,50.877 148.60097,0 c 25.2496,0 49.4977,18.3928 61.1778,33.0078 11.68,14.6148 21.9097,33.8111 22.2441,54.1699 l 0.7715,46.916 -4.4707,-14.0507 -24.0508,0 0,16.7773 c -22.0508,-55.0029 -75.3353,-91.0677 -134.5937,-91.0976 -80.12875,0 -145.08594,64.9572 -145.08597,145.0859 3e-5,80.1287 64.95722,145.0859 145.08597,145.0859 59.2888,-0.05 112.5819,-36.1694 134.5937,-91.2207 l 0,10.4239 24.0508,0 6.4746,-23.125 0,-3.0157 26.8965,-0.055 3.5351,-23.8964 -2.164,-120.7969 c -0.7871,-39.7102 -8.7191,-66.9314 -27.5762,-89.6777 -21.8149,-26.3144 -75.9882,-44.977 -103.7737,-45.3887 l 0,-52.1884 33.2073,16.536 c 36.1492,4.8545 69.8187,24.368 95.4082,53.4414 73.7355,16.928 130.3073,41.6911 184.1895,62.8497 6.5031,3.4825 14.3708,5.5234 22.8515,5.5234 22.3472,0 40.4629,-14.1499 40.4629,-31.6035 0,-8.6696 -0.975,-24.8633 -7.9746,-31.6895 -5.1918,-5.063 -59.8009,-4.9748 -65.8262,0.6895 -1.9662,1.8484 -3.3784,4.2864 -4.4101,7.0215 -74.7102,-32.7904 -143.039,-65.569 -181.0156,-119.3028 77.5063,-74.8526 193.5198,-123.84081 371.6074,-194.76561 l -0.092,-0.0332 c 21.0086,-6.68595 35.8242,-22.78639 35.8242,-41.59765 0,-12.3205 -1.3867,-35.33436 -11.334,-45.03516 -7.378,-7.1953 -84.9844,-7.06893 -93.5469,0.98047 -10.5333,9.9021 -10.125,31.51239 -10.125,44.05469 0,5.17928 1.1377,10.14792 3.2032,14.77734 -156.5149,53.43022 -288.9602,117.67582 -472.0625,117.67582 l -3.2696,0 c -183.10219,0 -315.54757,-64.2456 -472.06247,-117.67582 2.06544,-4.62942 3.20313,-9.59806 3.20313,-14.77734 0,-12.5423 0.40833,-34.15259 -10.125,-44.05469 -4.28127,-4.0247 -25.82496,-6.06902 -47.21875,-6.20703 z m 82.92578,240.33788 c -173.44528,-0.1323 -305.9272,46.5863 -309.40039,110.4082 -3.8534,70.8394 151.86466,136.9088 347.80664,147.5703 127.9877,6.8732 247.27619,-11.714 312.16602,-48.6406 -5.46184,-6.5906 -8.45766,-14.8778 -8.47266,-23.4375 l 0,-12.6504 c -11.91643,1.3673 -23.41097,2.9501 -34.48047,4.7441 -29.85813,28.8986 -97.94892,48.9755 -183.1543,54.004 -13.16604,5.2368 -26.1599,10.4791 -39.1582,15.5957 -11.33353,5.6514 -24.03269,8.6093 -37.31836,8.6093 -18.56075,0 -36.02775,-5.6386 -50.15625,-16.6738 -4.53804,-3.5445 -8.76524,-7.8209 -12.42187,-12.6738 -128.19115,-16.6082 -218.34973,-62.5862 -215.91407,-110.1094 2.80115,-51.4933 113.0483,-88.7421 255.04688,-86.1719 9.21785,0.167 18.46704,0.5027 27.71289,1.0059 56.02387,3.0872 110.36755,12.2356 155.87305,26.2402 3.23218,-2.6925 6.33699,-5.4232 9.29492,-8.2012 -14.90597,-11.9797 -31.36978,-23.4434 -49.50391,-34.664 -37.01445,-6.7444 -76.06948,-11.3104 -115.55469,-13.5098 -11.82896,-0.6432 -23.6621,-1.0721 -35.45507,-1.2851 -5.67731,-0.1028 -11.31515,-0.1559 -16.91016,-0.1602 z m 885.41601,0.014 c -4.1595,0.022 -8.3273,0.069 -12.5019,0.1445 -11.7931,0.2137 -23.6262,0.6433 -35.4551,1.2871 -39.4769,2.1963 -78.5252,6.7584 -115.5352,13.4981 -18.1418,11.2244 -34.6121,22.6916 -49.5234,34.6757 2.9248,2.7469 5.9924,5.4481 9.1855,8.1114 45.5666,-13.9813 99.949,-23.0985 155.9824,-26.1504 9.246,-0.5032 18.495,-0.8389 27.7129,-1.0059 141.9986,-2.5702 252.2458,34.6786 255.0469,86.1719 2.5649,47.5642 -87.663,93.6058 -215.9922,110.2168 -3.6383,4.8093 -7.8387,9.0477 -12.3437,12.5664 -14.1285,11.0352 -31.5955,16.6738 -50.1563,16.6738 -13.2856,0 -25.9848,-2.9579 -37.3183,-8.6093 -13.0945,-5.1545 -26.1825,-10.4375 -39.4493,-15.7129 -35.3933,-2.0967 -68.3563,-6.8297 -96.9589,-13.9219 2.5201,10.3096 4.2291,21.1111 5.2246,32.3574 54.4435,8.3541 115.859,10.9965 178.084,7.6621 195.942,-10.6615 351.66,-76.7309 347.8066,-147.5703 -3.3939,-62.4283 -130.6163,-109.0264 -301.3574,-110.3789 -4.1405,-0.033 -8.2917,-0.037 -12.4512,-0.016 z m -441.2734,253.7168 c 67.9194,-5e-4 122.979,55.0591 122.9785,122.9785 -6e-4,67.9186 -55.0599,122.9771 -122.9785,122.9766 -67.91786,-6e-4 -122.97603,-55.0587 -122.97659,-122.9766 -4.9e-4,-67.9186 55.05798,-122.9779 122.97659,-122.9785 z m 0,24.832 c -54.20437,3e-4 -98.14531,43.9421 -98.14456,98.1465 3.5e-4,54.2036 43.94097,98.1442 98.14456,98.1445 54.2036,-4e-4 98.1441,-43.9409 98.1445,-98.1445 8e-4,-54.2043 -43.9402,-98.1461 -98.1445,-98.1465 z m -1.6739,7.5899 c 21.3193,0.1392 40.4446,9.3561 50.3067,26.5136 16.2883,28.3378 -20.6126,28.455 -55.5879,48.5586 -34.97532,20.1038 -54.78196,52.5819 -71.07032,24.2442 -16.28834,-28.3377 -1.13932,-67.6074 33.83594,-87.711 13.11572,-7.5388 27.15798,-11.3127 40.44528,-11.5898 0.6921,-0.014 1.3826,-0.02 2.0703,-0.016 z"
       style="color:#000000;display:inline;overflow:visible;visibility:visible;opacity:1;fill:#000000;fill-opacity:1;fill-rule:nonzero;stroke:none;stroke-width:8;stroke-linecap:round;stroke-linejoin:round;stroke-miterlimit:4;stroke-dasharray:none;stroke-dashoffset:0;stroke-opacity:0.59607843;marker:none;enable-background:accumulate"
       inkscape:connector-curvature="0" />
  </g>
</svg>

